A multigrid/ensemble Kalman Filter strategy for assimilation of unsteady flows

A sequential estimator based on the Ensemble Kalman Filter for Data Assimilation of fluid flows is presented in this research work. The main feature of this estimator is that the Kalman filter update, which relies on the determination of the Kalman gain, is performed exploiting the algorithmic features of the numerical solver employed as a model. More precisely, the multilevel resolution associated with the multigrid iterative approach for time advancement is used to generate several low-resolution numerical simulations. These results are used as ensemble members to determine the correction via Kalman filter, which is then projected on the high-resolution grid to correct a single simulation which corresponds to the numerical model. The assessment of the method is performed via the analysis of one-dimensional and two-dimensional test cases, using different dynamic equations. The results show an efficient trade-off in terms of accuracy and computational costs required. In addition, a physical regularization of the flow, which is not granted by classical KF approaches, is naturally obtained owing to the multigrid iterative calculations. The algorithm is also well suited for the analysis of unsteady phenomena and, in particular,for potential application to in-streaming Data Assimilation techniques.

==> App1.tex <==
\section{Results}
\label{sec:state_space_model}

%The compressible Navier--Stokes equations for Newtonian fluids. The equations are rewritten using the perfect gas law:
%\begin{eqnarray}
%    P&=&(E-0.5(u^2+v^2))\rho(\gamma-1)\label{eq:2DNS_GASLAW_P}\\
%    T&=&\frac{\gamma}{\gamma-1}\frac{P}{Cp\cdot\rho},\label{eq:2DNS_GASLAW_T}
%\end{eqnarray}
%from which we obtain the continuity equation
%\begin{equation}
%\frac{\partial \rho}{\partial t}= -\bigg(\frac{\partial \rho u}{\partial x}+\frac{\partial \rho v}{\partial y} \bigg),\label{eq:2DNS_CONT}
%\end{equation}
%the conservation of momentum in the horizontal direction
%\begin{eqnarray}
%\frac{\partial (\rho u)}{\partial t}& = &-(\gamma-1)\bigg(\frac{\partial (\rho E)}{\partial \nonumber x}-\frac{1}{2}\frac{\partial ((\rho u)u)}{\partial x}-\frac{1}{2}\frac{\partial ((\rho v)v)}{\partial x}\bigg)-\frac{\partial ((\rho u)u)}{\partial x}\\&&-\frac{\partial ((\rho u) v)}{\partial y}+\rho\nu\bigg(\frac{4}{3}\frac{\partial^2 u}{\partial x}+\frac{\partial^2 u}{\partial  y^2}+\frac{1}{3}\frac{\partial^2 v}{\partial x \partial y} \bigg),\label{eq:2DNS_MOMX}
%\end{eqnarray}
%the conservation of momentum in the vertical direction
%\begin{eqnarray}
%\frac{\partial (\rho v)}{\partial t}&= &-(\gamma-1)\bigg(\frac{\partial (\rho E)}{\partial \nonumber y}-\frac{1}{2}\frac{\partial ((\rho u)u)}{\partial y}-\frac{1}{2}\frac{\partial ((\rho v)v)}{\partial y}\bigg)-\frac{\partial ((\rho v)v)}{\partial y}\\&&-\frac{\partial ((\rho u) v)}{\partial x}+\rho\nu\bigg(\frac{4}{3}\frac{\partial^2 v}{\partial y^2}+\frac{\partial^2 v}{\partial x^2}+\frac{1}{3}\frac{\partial^2 u}{\partial x \partial y} \bigg), \label{eq:2DNS_MOMY}
%\end{eqnarray}
%and finally, the conservation of energy
%
%\begin{eqnarray}
%\frac{\partial (\rho E)}{\partial t}&=&-\frac{\partial ((\rho E) u)}{\partial x} \nonumber
%-(\gamma-1)\bigg(\frac{\partial ((\rho E) u)}{\partial x}
%+\frac{1}{2}\frac{\partial ((\rho u)u^2)}{\partial x}
%+\frac{1}{2}\frac{\partial ((\rho v)v u)}{\partial x}\bigg)
%\\&&-\frac{\partial ((\rho E) v)}{\partial y}-(\gamma-1)\bigg(\frac{\partial ((\rho E) v)}{\partial y} \nonumber
%+\frac{1}{2}\frac{\partial ((\rho u)u v)}{\partial y}
%+\frac{1}{2}\frac{\partial ((\rho v) v^2)}{\partial x}\bigg)\\&&
%+\alpha\gamma\bigg(\frac{\partial^2 (\rho E )}{\partial x^2}
%-\frac{1}{2}\frac{\partial^2 ((\rho u)u )}{\partial x^2} \nonumber
%-\frac{1}{2}\frac{\partial^2 ((\rho v)v )}{\partial x^2}\bigg)\\&&
%+\alpha\gamma\bigg(\frac{\partial^2 (\rho E )}{\partial y^2}\nonumber
%-\frac{1}{2}\frac{\partial^2 ((\rho u)u )}{\partial y^2}
%-\frac{1}{2}\frac{\partial^2 ((\rho v)v )}{\partial y^2}\bigg)\\&&+(\rho u) \nu\bigg(\frac{4}{3}\frac{\partial^2 u}{\partial x^2} \nonumber
%+\frac{\partial^2 u}{\partial y^2}
%+\frac{1}{3}\frac{\partial^2 v}{\partial x \partial y} \bigg)
%+(\rho v) \nu\bigg(\frac{4}{3}\frac{\partial^2 v}{\partial y^2}
%+\frac{\partial^2 v}{\partial x^2}
%+\frac{1}{3}\frac{\partial^2 u}{\partial x \partial y} \bigg)\\&&+2\rho \nu\bigg[\bigg(\frac{\partial u}{\partial x} \bigg)^2 
%+\bigg(\frac{\partial v}{\partial y} \bigg)^2 \bigg]
%-\frac{2}{3}\rho \nu\bigg(\frac{\partial u}{\partial x} 
%+\frac{\partial v}{\partial y}  \bigg)^2
%+\rho \nu\bigg(\frac{\partial u}{\partial y} 
%+\frac{\partial v}{\partial x}  \bigg)^2
%\end{eqnarray}
\begin{figure}
\centering
\includegraphics[width=1\textwidth]{figures/mxl_t11_truth.png}
\caption{\label{fig:2D-mxl-trutht11}Flow calculated using a 2D Navier-Stokes equation. Visualization of the normal velocity field for the reference simulation for $t=11t_c$.}
\end{figure}

\begin{figure}
  \begin{subfigure}{\textwidth}
  \includegraphics[width=1\linewidth]{figures/MGENKF_rc4_t1_mxl.png}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\textwidth}
  \includegraphics[width=1\linewidth]{figures/MGENKF_rc4_t5_mxl.png}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\textwidth}
\includegraphics[width=1\linewidth]{figures/MGENKF_rc4_t33_mxl.png}
  \end{subfigure}
  \caption{\label{fig:MGENKF_states_rc4} Time evolution of the quantity $\rho v$ at the centerline of the mixing layer, calculated using the Multigrid EnKF (MEnKF) estimator. The case for $r_C=4$ is here shown. Total simulation time of $t=1$, $t=5$ and $t=33$ (in $t_c$ units) for state (a), (b) and (c), respectively. The blue line represents the True state, the orange line is the estimator and the red line is the EnKF correction. }
\end{figure}

\begin{figure}
  \begin{subfigure}{\textwidth}
  \includegraphics[width=1\linewidth]{figures/MGENKF_rc4_t1_mxl.png}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\textwidth}
  \includegraphics[width=1\linewidth]{figures/MGENKF_rc4_t5_mxl.png}
  \end{subfigure}\par\medskip
  \begin{subfigure}{\textwidth}
\includegraphics[width=1\linewidth]{figures/MGENKF_rc4_t33_mxl.png}
  \end{subfigure}
  \caption{\label{fig:MGENKF_states_rc4} Time evolution of the quantity $\rho v$ at the centerline of the mixing layer, calculated using the Multigrid EnKF (MEnKF) estimator. The case for $r_C=4$ is here shown. Total simulation time of $t=1$, $t=5$ and $t=33$ (in $t_c$ units) for state (a), (b) and (c), respectively. The blue line represents the True state, the orange line is the estimator and the red line is the EnKF correction. }
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\textwidth]{figures/stats_DENKF_mxl.png}
\caption{\label{fig:stats_DENKF_mxl}Root Mean Square Error RMSE integrated over the whole physical domain for $r_C=4$.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\textwidth]{figures/param_avg_DENKF_mxl}
\caption{\label{fig:param_DENKF_mxl}Parametric optimization of the value of $\epsilon_1$ to be applied at the inlet for the refined simulation.}
\end{figure} 

==> App2_Moldovan.tex <==
\section{Data Assimilation algorithm}
\label{sec:DA_algorithms}

%\begin{algorithm}
%   \SetKw{init}{Initialization}
%   \init $k:=0$; $\theta_0 = N(0, Q_\theta)$; $u(x,0)=u_0$; $u^{i}(x,0)=u_0$;  $i=1,...,N$; $\Phi=\Phi_0$\\
%   \While{$k<T$}{
%      Fine grid model integration:
%       $x_k^{f,F}=\mathcal{M}^F_{k:k-1}x_{k-1}^{a,F}$; $\mathcal{M}^F_{k:k-1}=\mathcal{M}^F_{k:k-1}\big(x_{k-1}^{a,F},\overline{\theta}_{k-1}^a\big)$\\  %$u(0,t)=u_0+\overline{a} sin(\omega t)$\\
%      Ensemble coarse model integration: $x_k^{f,C,(i)}=M_{k:k-1}^{C,(i)} x_{k-1}^{a,C,(i)}$; $M_{k:k-1}^{C,(i)}=M_{k:k-1}^{C,(i)}\big(x_{k-1}^{a,C,(i)},\theta_{k-1}^{a,(i)}\big)$\\
%      
%      Error inflation in the parameter: $\theta_k^{f,(i)}=\theta_{k-1}^{a,(i)}+\phi^{(i)}$, $\phi^{(i)}=N(0,\Phi)$\\
%      \If {Observation available}{
%      Calculation of statistics from the coarse state ensemble: $\overline{x}_k^{f,C}=\frac{1}{N}\sum_{n=1}^{N}x_k^{f,C,(i)} $; $X_k^C=\frac{1}{\sqrt{N-1}}\big[x_k^{f,C,(1)}-\overline{x}_k^{f,C},...,x_k^{f,C,(N)}-\overline{x}_k^{f,C}\big]$ \\
%      Calculation of statistics from the parameter ensemble:
%      $\overline{\theta}_k^f=\frac{1}{N}\sum_{n=1}^{N}\theta_k^{f,(i)} $; $\Theta_k=\frac{1}{\sqrt{N-1}}\big[\theta_k^{f,(1)}-\overline{\theta}_k^f,...,\theta_k^{f,(N)}-\overline{\theta}_k^f\big]$\\
%      Kalman Gain Calculation: $K_k^{e,C}=X_k^C Y^T(Y Y^T+R^C)^{-1}$; $K^{e,C,\theta}_k=\Theta_k Y^T(Y Y^T+R^C)^{-1}$; $Y=\mathcal{H}^C X_k^C$ \\
%      Creation of an ensemble of observations: $y_k^{o,C,(i)}=y_k^{o,C}+\epsilon^{C,(i)}$, $\epsilon^{C,(i)}=N(0,R^C)$\\
%      KF correction of the coarse ensemble state and parameter:  $x_k^{a,C,(i)}=x_k^{f,C,(i)}+K^{e,C}_k\big[y_k^{o,C,(i)}-\mathcal{H}^C x_k^{f,C,(i)}\big]$; $\theta_k^{a,(i)}=\theta_k^{f,(i)}+K^{e,C,\theta}_k\big[y_k^{o,C,(i)}-\mathcal{H}^C x_k^{f,C,(i)}\big]$\\
%
%	  Projection of the fine grid solution on the coarse grid $(x^{*})^{f,F}_k=J^C_F\big(x_k^{f,F}\big)$;\\
%	  Fine grid state corrected with the ensemble statistics $(x^{'})^F_k=x^f_k+J^F_C\big(K^{e,C}_k[y_k^{o,C}-\mathcal{H}(x^{*})^{f,F}_k]\big) $;\\         
%
%      Iterative procedure on the final solution:
%      %$\Psi_{k:k-1}^{'}u^a_k=\Psi_{k:k-1}u^{a}_{k-1}$, $\Psi_{k:k-1}=\Psi_{k:k-1}\big(u^{a}_{k-1},\overline{\theta}_{k-1}^a\big)$, $\Psi_{k:k-1}^{'}=\Psi_{k:k-1}^{'}\big(u^{'}_{k},\overline{\theta}_{k}^a\big)$ \\
%      $x^{a,F}_k=\alpha (x^{'})^F_k+\big(1-\alpha\big)\mathcal{M}^F_{k:k-1}x_{k-1}^{a,F}$; $\mathcal{M}^F_{k:k-1}=\mathcal{M}^F_{k:k-1}\big((x^{'})^F_k,\overline{\theta}_{k}^a\big)$\\}
%            $k:=k+1$;\\
%            
%   }
%   \caption{Multigrid EnKF algorithm.}
%   \label{alg:algo_iteratif_classique}
%\end{algorithm}

%\begin{algorithm}
%   \SetKw{init}{Initialization}
%   \init$\Big\{\theta_{0}^{a,(i)},\big(x_{0}^{a}\big)^F, \big(x_{0}^{a,(i)}\big)^C\Big\}$ with $i=1,...,N$;\\% $k:=0$; $\theta_0 \sim \mathcal{N}(0, Q_\theta)$; $(u)^F(x,0)=u_0$; $(u^{(i)})^C(x,0)=u_0$;  $i=1,...,N$; $\Phi=\Phi_0$\\
%   
%   \While{$k<T$}{
%      Parameter error inflation: $\theta_k^{f,(i)}=\theta_{k-1}^{a,(i)}+\tau^{(i)}_k$, $\tau^{(i)}_k\sim\mathcal{N}(0,\Sigma^{\theta}_k)$\\
%      Fine grid forecast:
%       $\big(x_k^{f}\big)^F=\mathcal{M}^F_{k:k-1}\Big(\big(x_{k-1}^{a}\big)^F,\overline{\theta}_{k-1}^a \Big)$;\\  %$u(0,t)=u_0+\overline{a} sin(\omega t)$\\
%      Ensemble coarse forecast: $\big(x_k^{f,(i)}\big)^C=\mathcal{M}_{k:k-1}^{(i),C}\Big(\big(x_{k-1}^{a,(i)}\big)^C,\theta_{k}^{f,(i)}\Big)$;\\
%     
%      \If {Observation available}{
%      Calculation of statistics from the coarse state ensemble: $\big(\overline{x}_k^{f}\big)^C=\frac{1}{N}\sum_{n=1}^{N}\big(x_k^{f,(i)}\big)^C $; $\big(X^f_k\big)^C=\frac{1}{\sqrt{N-1}}\Big[\big(x_k^{f,(1)}\big)^C-\big(\overline{x}_k^{f}\big)^C,...,\big(x_k^{f,(N)}\big)^C-\big(\overline{x}_k^{f}\big)^C\Big]$ \\
%      Calculation of statistics from the parameter ensemble:
%      $\overline{\theta}_k^f=\frac{1}{N}\sum_{n=1}^{N}\theta_k^{f,(i)} $; $\Theta^f_k=\frac{1}{\sqrt{N-1}}\Big[\theta_k^{f,(1)}-\overline{\theta}_k^f,...,\theta_k^{f,(N)}-\overline{\theta}_k^f\Big]$\\
%      Kalman Gain Calculation: $\big(K_k^{x,e}\big)^C=\big(X_k^f\big)^C Y_k^T(Y_k Y_k^T+R_k^C)^{-1}$; $\big(K^{\theta,e}_k\big)^C=\Theta^f_k Y_k^T(Y_k Y_k^T+R_k^C)^{-1}$; $Y_k=\mathcal{H}_k^C \big(X^f_k\big)^C$ \\
%      Creation of an ensemble of observations: $\big(y_k^{o,(i)}\big)^C=\big(y_k^{o}\big)^C+\big(\epsilon^{o,(i)}\big)^C$, $\big(\epsilon^{o,(i)}\big)^C \sim \mathcal{N}(0,R_k^C)$\\
%      KF correction of the coarse ensemble state and parameter:  $\big(x_k^{a,(i)}\big)^C=\big(x_k^{f,(i)}\big)^C+\big(K_k^{x,e}\big)^C\Big[\big(y_k^{o,(i)}\big)^C-\mathcal{H}_k^C \big(x_k^{f,(i)}\big)^C\Big]$; $\theta_k^{a,(i)}=\theta_k^{f,(i)}+\big(K_k^{\theta,e}\big)^C\Big[\big(y_k^{o,(i)}\big)^C-\mathcal{H}_k^C \big(x_k^{f,(i)}\big)^C\Big]$\\
%
%	  Projection of the fine grid solution on the coarse grid $\big(x^{*}_k\big)^C=\Pi^C_F\Big(\big(x_k^{f}\big)^F\Big)$;\\
%	  Fine grid state corrected with the ensemble statistics $\big(x^{'}_k\big)^F=\big(x_k^{f}\big)^F+\Pi^F_C\Big(\big(K_k^{x,e}\big)^C\Big[\big(y_k^{o}\big)^C-\mathcal{H}_k^C \big(x_k^{*}\big)^C\Big]\Big) $;\\         
%
%      Iterative procedure on the final solution:
%      %$\Psi_{k:k-1}^{'}u^a_k=\Psi_{k:k-1}u^{a}_{k-1}$, $\Psi_{k:k-1}=\Psi_{k:k-1}\big(u^{a}_{k-1},\overline{\theta}_{k-1}^a\big)$, $\Psi_{k:k-1}^{'}=\Psi_{k:k-1}^{'}\big(u^{'}_{k},\overline{\theta}_{k}^a\big)$ \\
%      $\big(x^{a}_k\big)^F=\alpha \big(x^{'}_k\big)^F+\big(1-\alpha\big)\mathcal{M}^F_{k:k-1}\Big(\big(x^{'}_k\big)^F, \big(x_k^{f}\big)^F, \overline{\theta}_k^a \Big)$;\\}
%            $k:=k+1$;\\
%            
%   }
%   \caption{Multigrid EnKF algorithm.}
%   \label{alg:algo_KF_corrected}
%\end{algorithm}

% Version Moldovan
\begin{algorithm}
   \SetKw{init}{Initialization}
   \init$\Big\{\theta_{0}^{a,(i)},\big(x_{0}^F\big)^a, \big(x_{0}^C\big)^{a,(i)}\Big\}$ with $i=1,...,N$;\\% $k:=0$; $\theta_0 \sim \mathcal{N}(0, Q_\theta)$; $(u)^F(x,0)=u_0$; $(u^{(i)})^C(x,0)=u_0$;  $i=1,...,N$; $\Phi=\Phi_0$\\
   
   \While{$k<T$}{
	
	Fine grid forecast:
       $\big(x_k^{F}\big)^f=\mathcal{M}^F_{k:k-1}\Big(\big(x_{k-1}^{F}\big)^a,\overline{\theta}_{k}^a \Big)$;\\  %$u(0,t)=u_0+\overline{a} sin(\omega t)$\\
      Parameter error inflation: $\theta_k^{f,(i)}=\theta_{k-1}^{a,(i)}+\tau^{(i)}_k$, $\tau^{(i)}_k\sim\mathcal{N}(0,\Sigma^{\theta}_k)$\\
      
      Ensemble coarse forecast: $\big(x_k^C\big)^{f,(i)}=\mathcal{M}_{k:k-1}^{C}\Big(\big(x_{k-1}^C\big)^{a,(i)},\theta_{k}^{f,(i)}\Big)$;\\
     
      \If {Observation available}{
	  Creation of an ensemble of observations: $\big(y_k^C\big)^{o,(i)}=\big(y_k^C\big)^{o}+\big(\epsilon^C\big)^{o,(i)}$, $\big(\epsilon^C\big)^{o,(i)} \sim \mathcal{N}(0,R_k^C)$\\
	  Compute normalized anomalies with $\big(y^C_k\big)^{f,(i)}$=$\mathcal{H}_k^C\Big( \big(x^C_k\big)^{f,i}\Big)$:\\
	  $\Big[\Theta^f_k\Big]_{:,i}=\frac{\theta^{f,(i)}_k-\overline{\theta^f_k}}{\sqrt{N-1}}$; $\Big[Y^f_k \Big]_{:,i}=\frac{\big(y^C_k\big)^{f,(i)}-\big(\overline{y^C_k}\big)^f}{\sqrt{N-1}}$\\
      $\theta$ Kalman Gain: $\big(K^C_k\big)^{\theta,e}=\Theta^f_k \big(Y_k^f\big)^T(Y_k^f \big(Y_k^f\big)^T+R_k^C)^{-1}$\\
      $\theta$ correction:
      $\theta_k^{a,(i)}=\theta_k^{f,(i)}+\big(K_k^C\big)^{\theta,e}\Big[\big(y_k^C\big)^{o,(i)}-\big(y^C_k\big)^{f,(i)}\Big]$\\
      Ensemble coarse forecast: $\big(x_k^C\big)^{f,(i)}=\mathcal{M}_{k:k-1}^{C}\Big(\big(x_{k-1}^C\big)^{a,(i)},\theta_{k}^{a,(i)}\Big)$;\\
      Compute normalized anomalies with $\big(y^C_k\big)^{f,(i)}$=$\mathcal{H}_k^C\Big( \big(x^C_k\big)^{f,i}\Big)$:\\
	  $\Big[\big(X^C_k\big)^f \Big]_{:,i}=\frac{\big(x^C_k\big)^{f,(i)}-\big(\overline{x^C_k}\big)^f}{\sqrt{N-1}}$; $\Big[Y^f_k \Big]_{:,i}=\frac{\big(y^C_k\big)^{f,(i)}-\big(\overline{y^C_k}\big)^f}{\sqrt{N-1}}$\\
	  $x$ Kalman Gain: $\big(K_k^C\big)^{x,e}=\big(X_k^C\big)^f Y_k^T(Y_k Y_k^T+R_k^C)^{-1}$\\
      $x$ correction: $\big(x_k^C\big)^{a,(i)}=\big(x_k^C\big)^{f,(i)}+\big(K_k^C\big)^{x,e}\Big[\big(y_k^C\big)^{o,(i)}-\big(y^C_k\big)^{f,(i)}\Big]$
      
      
      

	  Projection on the coarse grid $\left(x^{C}_k\right)^{*}=\Pi^F_C\left(\left(x_k^{F}\right)^f\right)$;\\
	  Fine grid state corrected with the ensemble statistics:\\
	  $\left(x^{C}_k\right)^{'}=\left(x^{C}_k\right)^{*}+\left(K_k^C\right)^{x,e}\left[\left(y_k^{C}\right)^o-\mathcal{H}_k^C\left(\left(x_k^{C}\right)^{*}\right)\right]$;\\
	  $\left(x^{F}_k\right)^{'}=\left(x_k^{F}\right)^f+\Pi^C_F\left(\left(x^{C}_k\right)^{'}-\left(x^{C}_k\right)^{*}\right) $;\\ 

      Matrix-Splitting iterative procedure on the final solution starting from $x_k^0=\big(x^{F}_k\big)^{'}$. 
			%Relaxation factor $\alpha=0.5$ used to obtain $\left(x^F_k\right)^a$
			}
      %$\Psi_{k:k-1}^{'}u^a_k=\Psi_{k:k-1}u^{a}_{k-1}$, $\Psi_{k:k-1}=\Psi_{k:k-1}\big(u^{a}_{k-1},\overline{\theta}_{k-1}^a\big)$, $\Psi_{k:k-1}^{'}=\Psi_{k:k-1}^{'}\big(u^{'}_{k},\overline{\theta}_{k}^a\big)$ \\
 
      
            $k:=k+1$;\\
            
   }
   \caption{Multigrid EnKF algorithm.}
   \label{alg:algo_KF_corrected_corrected}
\end{algorithm}

The algorithm \ref{alg:algo_KF_corrected_corrected} represents a simplified, ready-to-use application of the conceptual methodology presented in section \ref{sec:multigrid-EnKF}. This algorithm was tailored for the relatively simple physical models used in the present work. While it may not be suited for complex three-dimensional applications, it proved an optimum trade off in accuracy and computational resources for the present analysis. 

First of all, when observation is not available, the two main forecast operations (fine grid forecast and ensemble coarse forecast) are performed using explicit time advancement schemes. This choice allows to reduce the computational costs. However, when observation is available, the following strategies are employed: 
\begin{enumerate}
\item The two forecast operations (main simulation and ensemble members) are performed using an implicit matrix-splitting iterative procedure, using a single iteration. As stated in section \ref{sec:multigrid-EnKF}, the state matrices for each ensemble member are determined independently, but using the same structure and discretization schemes of the main simulation. 
%\item The forecast of the fine grid state and coarse grid ensemble (steps $1$ and $3$ of the conceptual algorithm) is performed using explicit time-integration procedures which, nonetheless, can be straightforwardly generalized to implicit time-integration schemes. In this explicit context $\delta=0$.
\item The number of iterative solutions for the main simulation on the coarse-grid level is equal to zero. That is, the solution from the first forecast is projected on the coarse grid, and the difference between the KF state estimation and this forecast is re-projected over the fine grid.
%\item The forecast of the ensemble members (step $3$ of the algorithm in section \ref{sec:multigrid-EnKF}) is performed explicitly, that is the state matrices $\left(\Psi\right)_k^{C,(i)}$ are unique to each member of the ensemble $\left(\Psi\right)_k^{C,(i)}=\left(\Psi\right)_k^{C,(i)}\left(\left(\mathbf{x}^C_{k-1}\right)^{a,(i)}\right)$. The test-cases where the algorithm has been tested do not necessarily require that $\left(\Psi\right)^C=\left(\Psi\right)^C\left(\left(\mathbf{x}^C_{k}\right)^{*}\right)$ is used for the construction of $\left(\Psi\right)_k^{C,(i)}$. The actual methodology required for doing this is under research. 
\item In the final iteration on the fine grid, an implicit matrix-splitting iterative procedure is employed, using a single iteration and a relaxation coefficient $\alpha=0.5$. This choice, which provides the best compromise between accuracy and regularization, has been identified after extensive tests for the configurations investigated.
%\item In the conceptual algorithm, $\left(x^{C}_k\right)^{'}$, is calculated iteratively by time-integrating $\left(x^{C}_k\right)^{*}$ with an implicit scheme. Assuming small $\Delta t$, $\left(x^{C}_k\right)^{'}$ can be directly calculated in a Kalman Filter fashion:$\left(x^{C}_k\right)^{'}=\left(x^{C}_k\right)^{*}+\left(K_k^C\right)^{x,e}\left[\left(y_k^{C}\right)^o-\mathcal{H}_k^C\left(\left(x_k^{C}\right)^{*}\right)\right]$. Note that by doing this the correction on the fine grid is not necessarily constrained and the smoothness of the solution will depend on the quality of the Kalman Gain operator $\left(K_k^C\right)^{x,e}$. 
  

\end{enumerate}

==> Cordier_Algorithm/Multigrid_EnKF_Moldovan.tex <==
% Version Moldovan original saved.
\begin{algorithm}
   \SetKw{init}{Initialization}
   \init$\Big\{\theta_{0}^{a,(i)},\big(x_{0}^F\big)^a, \big(x_{0}^C\big)^{a,(i)}\Big\}$ with $i=1,...,N$;\\% $k:=0$; $\theta_0 \sim \mathcal{N}(0, Q_\theta)$; $(u)^F(x,0)=u_0$; $(u^{(i)})^C(x,0)=u_0$;  $i=1,...,N$; $\Phi=\Phi_0$\\
   
   \While{$k<T$}{
	
	Fine grid forecast:
       $\big(x_k^{F}\big)^f=\mathcal{M}^F_{k:k-1}\Big(\big(x_{k-1}^{F}\big)^a,\overline{\theta}_{k}^a \Big)$;\\  %$u(0,t)=u_0+\overline{a} sin(\omega t)$\\
      Parameter error inflation: $\theta_k^{f,(i)}=\theta_{k-1}^{a,(i)}+\tau^{(i)}_k$, $\tau^{(i)}_k\sim\mathcal{N}(0,\Sigma^{\theta}_k)$\\
      
      Ensemble coarse forecast: $\big(x_k^C\big)^{f,(i)}=\mathcal{M}_{k:k-1}^{C}\Big(\big(x_{k-1}^C\big)^{a,(i)},\theta_{k}^{f,(i)}\Big)$;\\
     
      \If {Observation available}{
	  Creation of an ensemble of observations: $\big(y_k^C\big)^{o,(i)}=\big(y_k^C\big)^{o}+\big(\epsilon^C\big)^{o,(i)}$, $\big(\epsilon^C\big)^{o,(i)} \sim \mathcal{N}(0,R_k^C)$\\
	  Compute normalized anomalies with $\big(y^C_k\big)^{f,(i)}$=$\mathcal{H}_k^C\Big( \big(x^C_k\big)^{f,i}\Big)$:\\
	  $\Big[\Theta^f_k\Big]_{:,i}=\frac{\theta^{f,(i)}_k-\overline{\theta^f_k}}{\sqrt{N-1}}$; $\Big[Y^f_k \Big]_{:,i}=\frac{\big(y^C_k\big)^{f,(i)}-\big(\overline{y^C_k}\big)^f}{\sqrt{N-1}}$\\
      $\theta$ Kalman Gain: $\big(K^C_k\big)^{\theta,e}=\Theta^f_k \big(Y_k^f\big)^T(Y_k^f \big(Y_k^f\big)^T+R_k^C)^{-1}$\\
      $\theta$ correction:
      $\theta_k^{a,(i)}=\theta_k^{f,(i)}+\big(K_k^C\big)^{\theta,e}\Big[\big(y_k^C\big)^{o,(i)}-\big(y^C_k\big)^{f,(i)}\Big]$\\
      Ensemble coarse forecast: $\big(x_k^C\big)^{f,(i)}=\mathcal{M}_{k:k-1}^{C}\Big(\big(x_{k-1}^C\big)^{a,(i)},\theta_{k}^{a,(i)}\Big)$;\\
      Compute normalized anomalies with $\big(y^C_k\big)^{f,(i)}$=$\mathcal{H}_k^C\Big( \big(x^C_k\big)^{f,i}\Big)$:\\
	  $\Big[\big(X^C_k\big)^f \Big]_{:,i}=\frac{\big(x^C_k\big)^{f,(i)}-\big(\overline{x^C_k}\big)^f}{\sqrt{N-1}}$; $\Big[Y^f_k \Big]_{:,i}=\frac{\big(y^C_k\big)^{f,(i)}-\big(\overline{y^C_k}\big)^f}{\sqrt{N-1}}$\\
	  $x$ Kalman Gain: $\big(K_k^C\big)^{x,e}=\big(X_k^C\big)^f Y_k^T(Y_k Y_k^T+R_k^C)^{-1}$\\
      $x$ correction: $\big(x_k^C\big)^{a,(i)}=\big(x_k^C\big)^{f,(i)}+\big(K_k^C\big)^{x,e}\Big[\big(y_k^C\big)^{o,(i)}-\big(y^C_k\big)^{f,(i)}\Big]$
      
      
      

	  Projection on the coarse grid $\left(x^{C}_k\right)^{*}=\Pi^F_C\left(\left(x_k^{F}\right)^f\right)$;\\
	  Fine grid state corrected with the ensemble statistics:\\
	  $\left(x^{C}_k\right)^{'}=\left(x^{C}_k\right)^{*}+\left(K_k^C\right)^{x,e}\left[\left(y_k^{C}\right)^o-\mathcal{H}_k^C\left(\left(x_k^{C}\right)^{*}\right)\right]$;\\
	  $\left(x^{F}_k\right)^{'}=\left(x_k^{F}\right)^f+\Pi^C_F\left(\left(x^{C}_k\right)^{'}-\left(x^{C}_k\right)^{*}\right) $;\\ 

      Matrix-Splitting iterative procedure on the final solution starting from $x_k^0=\big(x^{F}_k\big)^{'}$. 
			%Relaxation factor $\alpha=0.5$ used to obtain $\left(x^F_k\right)^a$
			}
      %$\Psi_{k:k-1}^{'}u^a_k=\Psi_{k:k-1}u^{a}_{k-1}$, $\Psi_{k:k-1}=\Psi_{k:k-1}\big(u^{a}_{k-1},\overline{\theta}_{k-1}^a\big)$, $\Psi_{k:k-1}^{'}=\Psi_{k:k-1}^{'}\big(u^{'}_{k},\overline{\theta}_{k}^a\big)$ \\
 
      
            $k:=k+1$;\\
            
   }
   \caption{Multigrid EnKF algorithm.}
   \label{alg:algo_KF_corrected_corrected}
\end{algorithm}

==> Reserve/Sec2_copy_before_notation_change.tex <==
%\section{Model equations \& sequential state estimation}
\section{Sequential data assimilation in fluid dynamics}
\label{sec:maths}

In Section \ref{sec:discrEq}, we detail the steps that are necessary to transform a general transport equation into a discretized model 
usable in sequential DA. 
A brief description of the multigrid approach employed is provided. In Section \ref{sec:kalmanfilter}, the integration of such dynamical models in Kalman filtering procedures is discussed.

\subsection{From transport equation to multigrid resolution}
\label{sec:discrEq}

The general expression for a conservation equation in local formulation over a continuous physical domain reads as:
\begin{equation}
\rho \frac{\mathrm{D} \mathbf{x}}{\mathrm{D} t} = \nabla \cdot \overline{\overline{\sigma}} + \rho \mathbf{f} 
\label{eq:genConsEq}
\end{equation} 

where $\rho$ is the density of the flow and $\mathrm{D} / \mathrm{D}t$ is the total (or material) derivative of the physical quantity of investigation $\mathbf{w}$. The divergence operator is indicated as $\nabla \cdot$ while $\overline{\overline{\sigma}}$ is the stress tensor. Finally, $\mathbf{f}$ represents the effects of volume forces. The evolution of the flow is obtained via time advancement of the discretized solution, which is performed in a physical domain where initial and boundary conditions are provided. A general expression of the discretized form of  \eqref{eq:genConsEq} for the time advancement from the step $k-1$ to $k$ is given by:
\begin{equation}
\mathbf{x}_k = \Phi_k \mathbf{x}_{k-1} + B_k \mathbf{b}_k
\label{eq:generalDiscretizedForm}
\end{equation}

where $\Phi_k$ is the \emph{state matrix} which includes the discretized information of  \eqref{eq:genConsEq}. In case of non-linear dynamics described by \eqref{eq:genConsEq}, the state-of-the-art algorithms used for the discretization process are able to preserve the non-linear information in the product $\Phi_k \mathbf{x}_{k-1}$, up to a discretization error which is usually proportional to the size of the time step. The term $\mathbf{b}_k$ represents a \textit{controller} (such as for example boundary conditions) affecting the evolution of the physical quantity $\mathbf{x}$ via the matrix $B_k$. Bold characters denote vectors but the equations can be applied as well to scalar physical variables (such as the pressure $p$). Equation \eqref{eq:generalDiscretizedForm} is consistent with a time explicit discretization of \eqref{eq:genConsEq}. It is well known that this class of methods, despite the very high accuracy, may exhibit some unfavorable characteristics for the simulation of complex flows, such as limitations to the time step according to the Courant-Friedrichs-Lewy (CFL) condition \cite{Ferziger2002_springer}. One possible alternative to bypass this problem consists in using implicit schemes for time discretization. In this framework, the general structure of the discretized problem is usually cast in the form:   
\begin{equation}
\Psi_k \mathbf{x}_k = \widetilde{\Psi}_k \mathbf{x}_{k-1} + \widetilde{B}_k \mathbf{b}_k = \mathbf{c}_k
\label{eq:generalDiscretizedFormInt}
\end{equation}

where $\Psi_k$, $\widetilde{\Psi}_k$  and $\widetilde{B}_k$ are matrices obtained via the discretization process. Obviously, considering $\Phi_k = \Psi_k^{-1} \widetilde{\Psi}_k$, we retrieve \eqref{eq:generalDiscretizedForm}. However, this kind of manipulation is in practice not performed due to the prohibitive costs associated to large scale matrices inversions at each time step. Instead, iterative resolutions are usually employed to provide fast calculations of the solution when using implicit schemes. 
\lc{à revoir après section KF pour articulation}
Iterative solution rely on the progressive update of an initial solution provided until the residual $\delta$ (i.e. the error in the resolution of the algebraic scheme) is smaller than a prescribed threshold value. The procedure can be summarized as follows:
\begin{equation} 
\Psi_k \mathbf{x}_k^{1} = \mathbf{c}_k - \delta^{1} \;\; \to \;\; \Psi_k \mathbf{x}_k^{2} = \mathbf{c}_k - \delta^{2} \;\;\to \;\cdots\; \to \;\; \Psi_k \mathbf{x}_k^{n} = \mathbf{c}_k - \delta^{n} 
\label{eq:iterativeScheme}
\end{equation}

The number of iterations $n$ employed to reach convergence is determined by the condition $|\delta^{n}|<\epsilon$, where the tolerance $\epsilon$ is usually provided by the user. Among the several proposals in the literature, multigrid approaches are extensively used in CFD applications relying on iterative resolutions \cite{Hackbusch1985_springer,Ferziger2002_springer}. These methods generally iterate an initial solution on spaces characterized by a different level of resolution, which is then updated via multiple iterations to obtain the final solution on the computational grid. A common classification differentiate these tools in \textit{algebraic} multigrid and \textit{geometric} multigrid. The algebraic multigrid provides an initial estimation via manipulation / filtering of the state matrix $\Psi$. On the other hand, the geometric multigrid obtains the iterative solution via communication between two (or more) meshes. For the simpler case of two meshes that will be presented in the following, the grids will be referred to as $G$ and $\overline{G}$. The coarse-level grid $\overline{G}$ is usually obtained suppressing multiple mesh elements from the inital fine-level grid $G$. This operation is usually defined by a coarsening ratio, which indicates the total number of elements of $G$ over the number of elements conserved in $\overline{G}$. Among the numerous algorithms proposed for geometric multigrid application, the well-known Full Approximation Scheme (FAS) is a well documented strategy \cite{Brandt1977_mc,Wesseling1999_jcam}. A general formulation for a two-grid algorithm for the time step $k$ is now provided. The time subscript is excluded for clarity. Quantities under hat are defined in the coarse-grid space:
\begin{enumerate}
\item Starting from an initial solution on the fine grid $\mathbf{x}^0$ (which is usually equal to $\mathbf{x}_{k-1}$ in the first loop), an iterative procedure is applied to obtain a first solution $\mathbf{x}^1$. A residual $\delta= \mathbf{c}_k - \Psi_k \mathbf{x}^1$ is calculated.
\item $\mathbf{x}^1$ and $\delta$ are projected from the fine grid to the coarse grid space via a projection operator $\Pi^F_C$, so that $\overline{\mathbf{x}^1}$ and $\overline{\delta}$ are obtained. Similarly, the state matrix $\Psi$ is projected on the coarse grid to obtain $\overline{\Psi}$ and $\overline{\mathbf{c}}=\overline{\Psi} \, \overline{\mathbf{w}^1}+\overline{\delta}$.
\item An iterative procedure is employed to obtain $\overline{\mathbf{x}^2}$ on the coarse grid using as initial solution $\overline{\mathbf{x}^1}$.
\item The updated variable on the fine grid is obtained as $\mathbf{x}^2=\mathbf{x}^1+ \Pi^C_F\left(\overline{\mathbf{x}^2}-\overline{\mathbf{x}^1}\right)$. $\Pi^C_F$ is a projection operator from the coarse grid to the fine grid.
\item At last, the final solution $\mathbf{x}^3$ is obtained via a second iterative procedure on the fine grid starting from the intermediate solution $\mathbf{w}^2$. 
\end{enumerate}

This loop can be repeated multiple times imposing $\mathbf{x}^3=\mathbf{x}^0$ at the beginning of each cycle. When convergence is reached, $\mathbf{x}_k=\mathbf{x}^3$. Performing part of the calculations on a coarse grid level provides advantages for two aspects \cite{Ferziger2002_springer}. First, a significant reduction in the computational resources demanded is obtained when compared with full-matrix iterative procedures. The two projection operations via $\Pi^F_C$ and $\Pi^C_F$ plus the calculations performed over $\overline{G}$ are usually much less expensive than a full set of iterations over the grid $G$. Second, spurious high-frequency numerical oscillations due to the discretization error in $G$ are naturally filtered via the operators $\Pi^F_C$ and $\Pi^C_F$, which globally improves the quality of the numerical solution.

\subsection{Kalman Filter}
\label{sec:kalmanfilter}

The Kalman Filter (KF)  uses a system's dynamical model (e.g., first principle equations), a set of measurements or observations, and known control inputs to that system,  to provide an optimal state  estimation. Let us denote $\mathbf{x}_k$, the state of a physical system at time $k$. Similarly with the description given in Section \ref{sec:discrEq}, the state evolves from the instant $k-1$ to $k$ according to 
%\begin{equation}
%\mathbf{w}_{k}=\Phi_k \mathbf{w}_{k-1} + B_k \mathbf{c}_k + \mathbf{q}_k
%\label{eq:x_mdl}
%\end{equation}
\begin{equation}
\mathbf{x}_{k}=M_{k:k-1} \left(\mathbf{x}_{k-1}, \mathbf{\theta}_k\right)+\mathbf{q}_k
\label{eq:x_mdl}
\end{equation}

%where $\Phi_k$ is the state-transition linear model. Here,  $B_k$ is the control-input model which is applied to the control vector $\mathbf{c}_k$. 
where $M_{k:k-1}$ is a linear function acting as state-transition model and $\mathbf{\theta}_k$ contains the ensemble of parameters that influence the state-transition. The term $\mathbf{q}_k$ is associated with uncertainties in the model prediction which, as discussed before, could emerge for example from incomplete knowledge of initial / boundary conditions. In the framework of KF applications, these uncertainties are usually modelled as a zero-mean Gaussian distribution characterized by a variance $Q_k$, \textit{i.e.} $\mathbf{q}_k\sim\mathcal{N}(0,Q_k)$.

Discrete observations of $x_k$ are available in the components of the observation vector $y_k^o$ and related to the model state as:
%\begin{equation}
%\mathbf{z}_{k}=H_k \mathbf{x}_{k}+\mathbf{r}_k
%\label{eq:z_mdl}
%\end{equation}
\begin{equation}
\mathbf{y}_{k}^o=H_k\left( \mathbf{x}_{k}\right)+\mathbf{r}_k
\label{eq:z_mdl}
\end{equation}
where $H_k$ is the linear observation model which maps the model state space into the observed space. The available measurements are also affected by uncertainties which are assumed to follow a zero-mean Gaussian distribution characterized by a variance $R_k$, \textit{i.e.} $\mathbf{r}_k\sim\mathcal{N}(0,R_k)$.

%\rule{1cm}{1mm}

%In statistics and control theory, the Kalman Filter (KF) is a powerful algorithm used to integrate model prediction and measurements (observations) to provide an optimal state (in a given sense) estimation. Let us consider a variable $\mathbf{w}_k$ describing the state of a physical system at a time $k$. Similarly with the description presented in Section \ref{sec:discrEq}, the time evolution of the discretized system (\textit{model}) can be expressed by the equation:
%\begin{equation}
%\mathbf{w}_{k}=\Phi_k \mathbf{w}_{k-1} + B_k \mathbf{c}_k + \mathbf{q}_k
%\label{eq:x_mdl}
%\end{equation}

%where $\Phi_k$ is the state matrix used to advance in time the physical variable $\mathbf{w}$ from a instant $k-1$ to $k$. However, the term $\mathbf{q}_k$ is now included in the model. This term is associated with uncertainties in the model prediction which, as discussed before, could emerge for example from incomplete knowledge of initial / boundary conditions. In the framework of KF applications, these uncertainties are usually modelled as a zero-mean Gaussian distribution $\mathbf{q}_k=\mathcal{N}(0,Q_k)$ characterized by a variance $Q_k$. Similarly, available observation $\mathbf{z}_k$ at the time step $k$ is usually represented via the equation:
%\begin{equation}
%\mathbf{z}_{k}=H_k \mathbf{w}_{k}+\mathbf{r}_k
%\label{eq:z_mdl}
%\end{equation}
%where $H_k$ is the observation matrix. The available measurements also affected by epistemic uncertainty. This uncertainty is as well modelled using a zero-mean Gaussian distribution $\mathbf{r}_k=\mathcal{N}(0,R_k)$ characterized by a time-dependent variance $R_k$. 
Following the notation generally used in DA literature, the \textit{forecast}/\textit{analysis} states and error covariances are indicated as $\mathbf{x}^{f/a}_k$ and $\mathbf{P}^{f/a}_k$ respectively.  Starting from a forecast of the state $\mathbf{x}_k^f$ performed with the linear model $M_{k:k-1}$ and the previous known state, the Kalman Filter provides a State Estimation $\mathbf{x}_k^a$ manipulating the model and the observation, according to the level of confidence in each tool measured by $Q_k$ and $R_k$. The evolution in time of the global error of the system is stored in the error covariance matrix $\mathbf{P}^{f/a}_k=\mathbf{E}\left(\left(\mathbf{x}_k^{f/a} - \mathbf{E}\left(\mathbf{x}_k)\right)\right) \times \left(\mathbf{x}_k^{f/a} - \mathbf{E}\left(\mathbf{x}_k)\right)\right)^T \right)$ which is the essential element in the sequential process. As will be shown, $\mathbf{P}$ conserves the memory of the evolution of the estimated state from the initial condition to the time step $k$. The estimated state is obtained via a recursive procedure:  
\begin{enumerate}
  \item A predictor (forecast) phase, where the state of the system at a previous time-step is used  to obtain an \textit{a priori} estimation of the system at the current instant. This prediction, which is obtained relying on the model only, is not yet conditioned by observation at time $k$:
%\begin{eqnarray}
%\hat{\mathbf{w}}_{k|k-1}&=&\Phi_k\hat{\mathbf{w}}_{k-1|k-1}\label{eq:x_mdl_kf}\\
%P_{k|k-1}&=&\Phi_k P_{k-1|k-1} {\Phi_k}^T+Q_k \label{eq:P_mdl_kf}
%\end{eqnarray}
\begin{eqnarray}
\mathbf{x}^f_{k}&=&M_{k:k-1} \mathbf{x}^a_{k-1}\label{eq:x_mdl_kf}\\
\mathbf{P}^{f}_{k}&=&M_{k:k-1} \mathbf{P}^{a}_{k-1} {M_{k:k-1}}^T+Q_k \label{eq:P_mdl_kf}
\end{eqnarray}
  \item An update (analysis) step, where the state estimation is updated accounting for observation at the time $k$:
  %\begin{eqnarray}
  %K_k&=&P_{k|k-1}{H_k}^T(H_k P_{k-1|k} {H_k}^T+R_k)^{-1}\label{eq:k_kf}\\
  %\hat{\mathbf{w}}_{k|k}&=&\hat{\mathbf{w}}_{k|k-1} + K_k(\mathbf{z}_k-H_k\hat{\mathbf{w}}_{k|k-1})\label{eq:x_kf}\\
  %P_{k|k}&=&(I-K_k H_k)P_{k|k-1}\label{eq:P_kf}
  %\end{eqnarray}
   \begin{eqnarray}
  \mathbf{K}^x_k&=&\mathbf{P}^{f}_{k}{H_k}^T\left(H_k \mathbf{P}^{f}_{k} {H_k}^T+R_k\right)^{-1}\label{eq:k_kf}\\
  \mathbf{x}^a_{k}&=&\mathbf{x}^f_{k} + \mathbf{K}^x_k\left(\mathbf{y}^o_k-H_k\mathbf{x}^f_{k}\right)\label{eq:x_kf}\\
  \mathbf{P}^{a}_{k}&=&\left(I-\mathbf{K}^x_k H_k\right)\mathbf{P}^{f}_{k}\label{eq:P_kf}
  \end{eqnarray}
\end{enumerate}
The optimized prediction of the state $\mathbf{x}^a_{k}$ prediction is performed via a combination of model results and observation via the so called \textit{Kalman gain} $\mathbf{K}^x_k$. This operator combines the error information stored in $\mathbf{P}$ (which account for all the states before the time $k$) and the variances $Q_k$ and $R_k$. 
The classical KF algorithm is not suited for direct application to the analysis of complex flows. First of all, KF classical formulation is developed for linear systems. Applications to non-linear systems can be performed using more advanced techniques such as the extended Kalman filter \cite{Wan1997_adsy} or exploiting features of the numerical algorithms used for numerical discretization \cite{Meldi2017_jcp}. The components of the physical state $\mathbf{x}_k$ are arrays whose dimension $N \in [10^6, \, 10^9]$ in engineering applications. The matrices $Q_k$ and $R_k$ are usually unknown and their behavior must be modelled. One simple, classical simplification is to consider that uncertainties for each variable are completely uncorrelated in space and from other variables i.e. $Q_k$ and $R_k$ are considered to be diagonal \cite{Brunton2015_amr}. 
%In addition, the size of the error covariance matrix $P$ scales with $N^2$ and the \textit{a priori} estimation of the error covariance matrix scales with $N^3$ [REF???]. 
The computational cost associated with the application of a KF algorithm relying on a complete representation of $\mathbf{P}$ is thus unaffordable in practical applications due to the extensive manipulation (including inversion) of said matrix. One popular strategy to bypass the critical cost for the manipulation and storage of $\mathbf{P}$ is to rely on a statistical description obtained via an ensemble of numerical simulations. The Ensemble Kalman Filter (EnKF) \cite{Evensen2009_Springer}, introduced by Evensen in 1994 \cite{Evensen1994} relies on the representation of $\mathbf{P}$ by means of an ensemble. More precisely, the error covariance matrix is approximated using a finite ensemble of model states of size $N$. If the ensemble members are generated using stochastic Monte-Carlo sampling, the error in the approximation decreases with a rate of $\frac{1}{\sqrt{N}}$.  

Given an ensemble of model states at a certain instant, the ensemble matrix is defined as:
\begin{equation}
    E_k^{f/a}=\left[\mathbf{x}_k^{f/a,(1)},...,\mathbf{x}_k^{f/a,(N)}\right]\in\mathbb{R}^{m\times N} \label{eq:Ensemble_Matrix}
\end{equation}
The matrix $E_k^{f/a}$ contains $N$ $m$-dimensional vectors each one of them representing the state of a member in the ensemble. The ensemble mean $\overline{\mathbf{x}}_k^{f/a}$ is obtained as:
\begin{equation}
    \overline{\mathbf{x}}_k^{f/a}=\frac{1}{N}\sum^{N}_{i=1}\mathbf{x}_k^{f/a,(i)}, \label{eq:Ensemble_Mean}
\end{equation}
once the average state is obtained, the ensemble-anomaly matrix is defined as
\begin{equation}
    X_k^{f/a}=\frac{\left[\mathbf{x}_k^{f/a,(1)}-\overline{\mathbf{x}}_k^{f/a},...,\mathbf{x}_k^{f/a,(N)}-\overline{\mathbf{x}}_k^{f/a}\right]}{\sqrt{N-1}}\in\mathbb{R}^{m\times N}. \label{eq:Ensemble_Anomaly}
\end{equation}
An approximation of the error covariance matrix $\mathbf{P}$ can thus be defined via the information derived from the ensemble: 
\begin{equation}
    \mathbf{P}_k^{f/a,e}=X_k^{f/a} \times \left(X_k^{f/a}\right)^T\in\mathbb{R}^{m\times m}, \label{eq:Ensemble_P}
\end{equation}
where the subscript $e$ indicates that the matrix is not exact, but it is estimated using information obtained from the ensemble. Evensen showed \cite{Evensen1994} that the model propagation of the error statistics in \eqref{eq:P_mdl_kf} is equivalent to integrating each model state of the ensemble according to the state transition equations. Moreover, he showed that applying the classical KF to each member of the ensemble resulted in a correct mean and covariance of the ensemble, in agreement with \eqref{eq:P_kf}. Burgers et al. \cite{Burgers1998} further clarified that in order for the EnKF to be consistent with the classical KF, the observation must be considered as a random variable with an average corresponding to the observed value and a covariance $R$. Therefore, given the discrete observation vector at an instant $k$ $\mathbf{y}^o_k\in \mathbb{R}^{d}$ the ensemble of perturbed observations is defined as:
\begin{equation}
    \mathbf{y}_k^{o,(i)}=\mathbf{y}_k^o+\mathbf{\epsilon}_k^{o,(i)}, \hspace{1cm} 1\leq i \leq N, \label{eq:perturbed_y}
\end{equation}
and the normalized anomaly ensemble matrix of the observations can be defined as:
\begin{equation}
    E^o_k=\left[\mathbf{\epsilon}_k^{o,(1)},...,\mathbf{\epsilon}_k^{o,(N)}\right]\in\mathbb{R}^{d\times N}, \label{eq:observation_matrix}
\end{equation}
and the error covariance matrix of the measurement error can be redefined as
\begin{equation}
    R_k^e=E^o_k \times \left(E^o_k\right)^T\in\mathbb{R}^{d\times d}. \label{eq:observation_matrix_errorcov}
\end{equation}
Once all of the elements are obtained, the KF update is performed on each of the members of the ensemble as
\begin{equation}
\mathbf{x}_k^{a,(i)}=\mathbf{x}_k^{f,(i)}+\mathbf{P}_k^{f,e} H_k^T\left[H_k \mathbf{P}_k^{f,e} H_k^T + R_k^e\right]^{-1}\left[y_k^{o,(i)}-H_k\mathbf{x}^{f,(i)}_k\right].\label{eq:ensemble_update}
\end{equation}
As previously described, Evensen showed that the statistics of the updated ensemble members $\mathbf{x}_k^a$ are consistent with the ones obtained using a classical KF application. 

State-of-the-art approaches based on the EnKF are arguably the most advanced forms of State Estimation available in the field of DA methods. These techniques have been extensively applied in the last decade in meteorology and geosciences \cite{Asch2016_SIAM}. Applications in mechanics and engineering are much more recent, despite a rapid increase in the number of applications in the literature. Among those, studies dealing with wildfire propagation \cite{Rochoux2014_nhess}, combustion \cite{Labahn2019_pci}, turbulence modeling \cite{Xiao2016_jcp} and hybrid variational-EnKF methods \cite{Mons2019_jcp} have been reported. These applications reinforce the idea that approaches based on EnKF have a high investigative potential despite the highly non-linear, multiscale features of the flows studied by the fluid mechanics scientific community.

The EnKF methods can also be used to perform Statistical Inference of the free parameters describing the model. This operation optimizes the performance of the model in order to get closer to the flow prediction provided by the EnKF State Estimation. Among the different strategies that can be employed to this purpose, the Dual state-parameter  estimation with EnKF technique \cite{DENKF_MORADKHANI2005} is a well established technique. Each analysis phase, the set of free parameters $\theta_k$ in each member of the ensemble is updated following the classical KF equation:
\begin{equation}
\mathbf{\theta}_{k}^a=\mathbf{\theta}_{k}^f +K_k^{\theta,e}\left(\mathbf{y}_k^{o,(i)}-H_k \mathbf{x}_k^{f,i}\right),\label{eq:EnKF par correction}
\end{equation}
where $K_k^{\theta,e}$ is the Kalman gain responsible for correcting the parameter trajectories in the ensemble and is obtained as follows:
\begin{equation}
K_k^{\theta,e}=\Theta_k^f H_k^T\left(H_k \mathbf{P}_k^{f,e} H_k^T + R_k^e\right)^{-1},
\end{equation}

Here $\Theta_k^f$ represents the anomaly to the parameter average and it is calculated similarly to the term $X_k^f$ in equations \ref{eq:Ensemble_Mean} $\&$ \ref{eq:Ensemble_Anomaly}:
\begin{equation}
    \overline{\mathbf{\theta}}_k^{f/a}=\frac{1}{N}\sum^{N}_{i=1}\mathbf{\theta}_k^{f/a,(i)}, \label{eq:EnsembleA_Mean}
\end{equation}
and once the average state is obtained, the ensemble-anomaly matrix is defined as
\begin{equation}
    \Theta_k^{f/a}=\frac{\left[\mathbf{\theta}_k^{f/a,(1)}-\overline{\mathbf{\theta}}_k^{f/a},...,\mathbf{\theta}_k^{f/a,(N)}-\overline{\mathbf{\theta}}_k^{f/a}\right]}{\sqrt{N-1}}\in\mathbb{R}^{p\times N}. \label{eq:EnsembleA_Anomaly}
\end{equation} 

This technique allows to perform a recursive state estimation / parametric inference using the information from the ensemble members. 


==> Sec0.tex <==
\todo{Le fil conducteur du papier n'est pas clair à suivre. On a l'impression que tous les mots-clés ont été mis dans le titre : "intrusive", "multigrid" et "ensemble" (name dropping). Le caractère "intrusive" ou non doit être commenté. Ne serait-ce pas d'ailleurs "non intrusive" ! Je ne vois pas le caractère "intrusive" comme un avantage. Au niveau de l'organisation du papier, j'aurais envie de commencer par la description de KF, d'expliquer les limites dues au problème de grande taille puis d'introduire le multigrille comme un moyen d'économiser du temps de calcul. }

\lc{Si je ne me trompe pas, nous sommes passés dans les développements numériques d'une approche où le coeur était l'utilisation d'une stratégie multigrille (à deux grilles en l'occurence) pour KF à une stratégie reposant sur l'EnKF et sur l'utilisation des deux grilles. EnKF est déjà considéré dans la communauté DA comme une méthode permettant de réduire le coût de calcul en estimant la matrice de covariance via une méthode d'ensemble plutôt qu'en la transportant. Il faudrait donc a prori tester cette méthode sur une même grille et montrer quel est le nombre d'individu minimum qu'il faut considérer pour obtenir une bonne représentation de la matrice de covariance. Cela nous donnerait alors un cas de référence à partir duquel on pourrait envisager des comparaisons. La stratégie à deux grilles ne serait alors là que pour montrer que le coût de calcul est réduit ou qu'à un coût de calcul donné l'erreur d'estimation est la même. Est-ce là l'objectif ?}

\lc{Nous avons besoin (j'ai besoin) d'avoir une description claire et nette des tests numériques que Gabriel réalise. Gabriel a obtenu beaucoup de résultats mais il est souvent difficile de savoir dans quelles conditions les tests ont été réalisés. du coup, il est difficil en l'état de connecter les sections "méthode" des sections "application". Imaginons que nous nous concentrons d'abord sur une équation de Burgers comme dans la section 4. Quel est alors l'objectif de l'assimilation de données ? Coment l'équation de Burgers a été résolu. Tout cela doit être précisé.} 

==> additionalMaterialByGabriel.tex <==
\section{\textcolor{cyan}{I have not touched the article from here on}}
   

where $F^a$ and $F^v$ represent the advective and viscous terms, respectively. A general form of the discretized representation of equation \eqref{eq:burgers_compact} can be written as:
\begin{equation}
 u_{k}=u_{k-1}+F^a_x(u_{k-1})+F^v_x(u_{k-1})\label{eq:burgers_compact_discre}
\end{equation}
The multiple numerical flux terms that affect \eqref{eq:burgers_compact} ($F^a_x$ and $F^v_x$) can be assembled in a single term $\Phi_k$ and the discretized form of the equation is represented as:
\begin{equation}
 u_{k}=u_{k-1}+\Phi_k(u_{k-1})\label{eq:burgers_compact_discre_compact}
\end{equation}
Equation \eqref{eq:burgers_compact_discre_compact} is reminiscent of the dynamical systems used in control theory (REF). It should be noted that the term $\Phi_k$ represents the discretization strategy used, as well as the model in itself. All the different fluid dynamics models analysed in this work can be written following the general 
form described in \eqref{eq:burgers_compact_discre_compact}.











To address the computational cost limitations associated with the application of the KF to compressible flows it is necessary to resort to model reduction techniques. The two major model reduction modifications that we want to implement rely on the two following hypothesis:
\begin{enumerate}
    \item The grid resolutions used in the compressible flow simulation framework are often extremely fine, which is necessary to capture the complete dynamics of the physical system. However, the type of mesh resolutions attainable through experimental measurement, such as Particle Image Velocimetry (PIV) for example, is orders of magnitude lower [REF]. In addition, the large coherent flow structures captured through direct measurement, which dictate the global dynamics of the flow [REF and some more information, maybe interesting], are sufficiently well defined with coarser resolutions. In conclusion, there are strong arguments for the application of the KF algorithm in a multiple grid framework where the state transition calculations are performed in a fine grid and the statistical modifications of the flow are performed in a secondary coarser grid. [ADD a FIGURE MAYBE]
    \item Consider a compressible flow phenomena analysed under experimental considerations. Usually, the available measurement information is limited to an observation window that represents a small region of the complete physical system. Would this experimental data be integrated into a numerical simulation, it would still represent a relatively small region when compared to the computational domain. The application of the full KF would entail a complete representation of the error covariance matrix of the whole domain. In practical applications, this is rarely achievable; even the accurate representation of the error observation matrix, limited in size to the observation window, can be problematic. It is necessary to resort to physical considerations. In some dynamical systems, the variables become spatially uncorrelated beyond some characteristic separation. Consequently, there is a strong case for the brute truncation of the error covariance matrix. That is, the domain where the KF applies, or the error space, could be reduced drastically. In practice, the error space can be created around the observation window and its size should be defined taking into account the spatial correlation of the flow. Beyond the error space, the KF no longer modifies the flow. The idea presented here is analogous to the \textit{Covariance Localization} technique which has been used in EnKF estimators [REF].
\end{enumerate}
In conclusion, the reduced-order KF methodology that we implemented can be summarized into two main aspects: the usage of multiple grids, fine and coarse, and the truncation of the error covariance matrix by reducing the actual size of the error space.

Let us define two spaces or grids that describe the same physical phenomena $x_k$ at an instant $k$. Let $x_k$ on the first space be defined as $x_k^F$, where $F$ stands for the representation of the phenomena on the fine grid. Consider that the current time-step of the phenomena has been calculated from a previous instant $k-1$ with the state-transition model. Let $x_k$ on the second space be defined as a projection of the fine grid representation on the coarse grid $x_k^C=\Pi^{F\rightarrow C}(x_k^F)$, where $\Pi$ is a projection operator. Consider now that observation $z_k^C$ at an instant $k$ is available on a coarse grid and the KF is to be applied in order to correct the representation of the phenomena on the fine space $x^F_k$. Considering the hypothesis discussed in the previous paragraph, the framework now presented allows for the application of the KF on the coarse grid, where $x_k^C$ and $z_k^C$ are integrated and a KF estimate $\hat{x}_k$ is obtained. In practice, the developed Multiple Grid KF algorithm can be conceptualized as a two-phase process:
\begin{enumerate}
  \item A predictor phase, where the state of the system at a previous time-step is used to obtain an \textit{a priori} estimate at the current instant. The estimation of $x$ is performed on the fine grid while the estimation of the error covariance is performed on the coarse grid.
  \begin{eqnarray}
    &\hat{x}_{k|k-1}^F=\Phi_k^F\hat{x}_{k-1|k-1}^F\label{eq:x_mdl_kfmg}\\
    &\hat{x}_{k|k-1}^C=\Pi^{F\rightarrow C}(\hat{x}_{k|k-1}^F)\label{eq:x_pFCmg}\\
    &P_{k|k-1}^C=\Phi_k^C P_{k-1|k-1}^C {(\Phi_k^C)}^T+Q_k^C \label{eq:Pkfmg}
  \end{eqnarray}
  \item An update step, where observation is combined with the \textit{a priori} estimate to obtain an optimal \textit{a posteriori} prediction on the coarse grid:
  \begin{eqnarray}
    &K_k^C=P_{k|k-1}^C{(H_k^C)}^T(H_k^C P_{k|k-1}^C {(H_k^C)}^T+R_k^C)^{-1}\label{eq:K_kfmg}\\
    &\hat{x}_{k|k}^F=\hat{x}_{k|k-1}^F + \underbrace{\Pi^{C\rightarrow F}\big  (K_k^C(z_k^C-H_k^C\hat{x}_{k|k-1}^C)\big)}_\text{KF Correction}\label{eq:x_kfcmg}\\
    &P_{k|k}^C=(I^C-K_k^C H_k^C)P_{k|k-1}^C\label{eq:Pc_kfmg}
  \end{eqnarray}
\end{enumerate}
Note that the superscripts $F$ and $C$ indicate if the variable which they accompany is represented on the fine or the coarse grid, respectively. It is straightforward to recognize the canon form of the KF in the Multiple Grid KF algorithm that we present. The major difference is that the KF correction is calculated not on the same space as where the state-transition is performed, but on a projection of a coarser version of this space. The coarse KF correction is then projected back on the fine space.

Equation \eqref{eq:Pkfmg} describes the \textit{a priori} estimation of the error covariance matrix. As stated before, this matrix operation scales with $N_C^3$ where $N_C$ is the dimension of the state vector $x^C_k$. Even on the reduced-order framework that we propose, \eqref{eq:Pkfmg} is problematic in terms of computational cost. Moreover, the state-transition of the covariance is performed on a coarse space $\Phi_k^C$, and the discretization errors can be significant, disrupting the covariance propagation in the system. In addition, the model error covariance $Q_k^C$ is imperfectly known, and usually estimated as proportional to a coefficient multiplied by the identity matrix $I$. Finally, the state-transition operator remains highly non-linear. The sum of the aforementioned factors can potentially render the covariance estimation unstable and the development of spurious cross-correlations is inevitable. Some authors propose [REF] a fixed error covariance matrix, so that \eqref{eq:Pkfmg} becomes:
\begin{equation}
    P_{k|k-1}^C=\Phi_k^C P_{k-1|k-1}^C {(\Phi_k^C)}^T+Q_k^C \rightarrow P_{k|k-1}^C=P_{k-1|k}^C+Q_k^C\label{eq:P_kfmg_fixed}
\end{equation}
completely removing the propagation of the covariance with the state-transition matrix. On the one side, this simplification provides huge reductions in terms of computational cost. On the other side, the spatial action range (not sure if good term) of the KF completely depends on the proper definition of the model error covariance. 

A more elegant way to deal with the limitations concerning the propagation of the error covariance matrix is the Monte-Carlo approach proposed by Evensen (REF), the Ensemble Kalman Filter EnKF. The EnKF and its variants are nowadays amongst the most popular data-driven methods applied in high-dimensional systems (ref annual review 2018 evensen) and it has been successfully applied in different domains. It has been proven that the EnKF estimator can give reliable results with just $100$ particles, which make it extremely appealing for data-driven applications.



The Multiple-Grid KF algorithm described in equations \eqref{eq:x_mdl_kfmg}-\eqref{eq:Pc_kfmg} is used as a starting point and modified to integrate an ensemble of coarse realizations. The assimilation process is split into two sub-processes. On the first sub-process, the model forecast is propagated on the fine grid on a single simulation. If observations are available, the KF update is to be performed on a coarse grid, using the statistics ($P^e$ and $R^e$) obtained in the second sub-process.
\begin{eqnarray}
    \hat{x}_{k|k-1}^F=\Phi_k^F\hat{x}_{k-1|k-1}^F\label{eq:EnKF_mg_x_fine_prop}\\
    \hat{x}_{k|k-1}^C=\Pi^{F\rightarrow C}(\hat{x}_{k|k-1}^F)\label{eq:EnKF_mg_x_fine_prop_coarseproj}\\
    K_k^C=(P^e)_{k|k-1}^C{(H_k^C)}^T\big(H_k^C (P^e)_{k|k-1}^C {(H_k^C)}^T+(R^e)_k^C\big)^{-1}\label{eq:EnKF_mg_K_coarse}\\
    \hat{x}_{k|k}^F=\hat{x}_{k|k-1}^F + \Pi^{C\rightarrow F}\big  (K_k^C(z_k^C-H_k^C\hat{x}_{k|k-1}^C)\big)\label{eq:x_kfcmg}
  \end{eqnarray}
On the second sub-process, an ensemble of $N$ coarse grid realizations are propagated forward and the EnKF is applied systematically. In this first version of the algorithm, the first sub-process does not influence at all the EnKF, thus being completely independent. However, the EnKF provides a coarse error covariance estimate for the first sub-process. Each member $n$ of the ensemble is forward with its associated state transition matrix as
\begin{equation}
(\hat{x}_n)_{k|k-1}^C=(\Phi_n)_k^C(\hat{x}_n)_{k-1|k-1}^C\label{eq:EnKF_mg_x_ensemble_prop},
\end{equation}
and the forecast error covariance is approximated as defined in equations \eqref{eq:Ensemble_Matrix},\eqref{eq:Ensemble_Mean}, \eqref{eq:Ensemble_Anomaly} and \eqref{eq:Ensemble_P}
\begin{equation}
    (P^e)^C_{k|k-1}=(X^C_{k|k-1})(X^C_{k|k-1})^T. \label{eq:EnKF_mg_ensemble_cov}
\end{equation}
An ensemble of perturbed observations is constructed as described in equations \eqref{eq:perturbed_y}, \eqref{eq:observation_matrix} and \eqref{eq:observation_matrix_anomaly}. The error covariance matrix of the measurement error is defined with the normalized anomaly ensemble of the observations
\begin{equation}
    (R^e)^C_k=(Y_o^{'})^C_k((Y_o^{'})^C_k)^T, \label{eq:EnKF_mg_observation_matrix_errorcov}
\end{equation}
and each member of the ensemble is updated according to the classical KF method
\begin{eqnarray}
K^C_k=(P^e)_{k|k-1}^C{(H_k^C)}^T\big(H_k^C (P^e)_{k|k-1}^C {(H_k^C)}^T+(R^e)_k^C\big)^{-1},\label{eq_EnKF_mg_K_ensemble}\\
(\hat{x}_n)^C_{k|k}=(\hat{x}_n)^C_{k|k-1}+K^C_k[(y_n)^C_k-H^C_k (\hat{x}_n)^C_{k|k-1}].\label{eq:ensemble_update}
\end{eqnarray}
The forecast error covariance matrix $(P^e)^C_{k|k-1}$ is transferred every instant there is an observation to the first  sub-process, where the fine grid simulation is corrected with the error statistics calculated in the ensemble sub-process. If the analysis error covariance $(P^e)^C_{k|k}$ is required, it can be obtained from the ensemble, but it is not necessary for the algorithm to perform, as the error statistics are correctly characterized in the ensemble. 

  
 
\section{Reconstruction of the error covariance matrix via sparse data}
The estimate provided by the KF algorithm is subject to uncertainties. This implies that the true state of the physical phenomena $x^{true}_k$ is completely unknown and therefore, the error in $\hat{x}_{k|k}$ must be tracked in a probabilistic fashion. The associate estimate error $\hat{e}_{k|k}$ can be defined as the difference between the estimate $\hat{x}_{k|k}$ and the true state $x^{true}_k$ of the phenomena:
\begin{equation}
    \hat{e}_{k|k}=\hat{x}_{k|k}-x^{true}_k\label{eq:e_kf}
\end{equation}

There are two parameters that directly affect $\hat{e}_{k|k}$: the error statistics of the uncertainties associated with the state-transition model $w_k$ and of the measurement error $v_k$, as described in \eqref{eq:x_mdl} and \eqref{eq:z_mdl} respectively. Under the assumption that these error statistics can be described by Gaussian Probability Density Functions (PDF), $\hat{e}_{k|k}$ can be fully described by the characteristic expected value $\mathbb{E}[\cdot]$ and an error covariance model. Providing that the state-transition model is unbiased, $\mathbb{E}[\hat{e}_{k|k}]=0$ and the statistics of $\hat{e}_{k|k}$ are characterized by a positive definite, square-symmetric matrix of size $N\times N$ where $N$ is dimension of $\hat{x}_{k|k}$, which satisfies:
\begin{equation}
    P_{k|k}=\mathbb{E}[(\hat{x}_{k|k}-x^{true}_k)(\hat{x}_{k|k}-x^{true}_k)^T]=\mathbb{E}[(\hat{e}_{k|k})(\hat{e}_{k|k})^T]\label{eq:P_kf_def}
\end{equation}

$P_{k|k}$, or the error covariance matrix describes the probabilistic behavior of the error in the KF estimate $\hat{x}_{k|k}$. Assuming that both observation and model error can be described by Gaussian PDF it follows that the KF estimate $\hat{x}_{k|k}$ is a Gaussian process $\hat{x}_{k|k}\sim \mathcal{N}(x^{true}_k,P_{k|k})$ and $\hat{e}_{k|k}\sim \mathcal{N}(0,P_{k|k})$. The diagonal elements of $P_{k|k}$ represent the error variance of each element in the vector state estimate $\hat{x}_{k|k}$ and the off-diagonal terms describe the covariance of each pair of components in $\hat{x}_{k|k}$. The error covariance is of pivotal importance. It describes the error correlations in the system and is responsible for the transferring of information between the multiple components of the state vector. For example, in the framework of sequential data assimilation, an accurate and complete $P_{k|k}$ would allow the KF algorithm to correct variables that are not directly observed. The error correlations present in $P_{k|k}$ influence the calculation of the Kalman Gain, which in turn dictates how each observed component of the state vector is corrected and how they affect the correction of their zone of influence.

It is clear that using a fixed error covariance matrix, as defined in \eqref{eq:P_kfmg_fixed}, can substantially limit the potential of the KF. The estimation of the model error covariance matrix $Q_k$ remains one of the most complex aspects of data assimilation and an open challenge in the statistics and control scientific community. One of the simplest and most robust forms for $Q_k$, proposed by different authors (REF) is a diagonal form in which the model error statistics are characterized solely by the error variance of each component of the state vector. Therefore, in the absence of a state-transition model for $P_{k|k}$, the KF correction is limited to the observed variables.

Let us consider a physical phenomena $x_k$ that is analysed with numerical simulation techniques. Consider that the state transition model used is exact and the uncertainties associated with the analysis occur from the inexact specification of the initial and boundary conditions. Consider that local, unbiased but noisy observation is available and ready to be sequentially integrated in the numerical analysis through the KF. No prior information is available for the estimation of the error covariance matrix $P_{k|k}$ nor the model error covariance matrix $Q_k$ but, the measurement error variance $\sigma_z$ is known so that $R_k=\sigma_z I$. The estimation of the model covariance matrix $Q_k$ is problematic. The canon application of the KF requires that the model error follow a gaussian process $w_k\sim \mathcal{N}(0,Q_k)$. It is not true for the case described here as the numerical prediction is completely biased. Nonetheless, the KF can still be applied with a model error covariance matrix that represents as accurately as possible the bias inherent to the numerical prediction.

One possible way to overcome the bias is to take advantage of the available observation. A crude approximation of the error in the estimate would be:
\begin{equation}
    P_{k|k}=\mathbb{E}[(\hat{x}_{k|k}-z_k)(\hat{x}_{k|k
    }-z_k)^T]\label{eq:P_kf_def_z}
\end{equation}
Nonetheless the available observation is limited to a local region of the analysis domain and thereby, the direct influence of the KF is limited to this region since the error covariance matrix is considered to be fixed \eqref{eq:P_kfmg_fixed}. However, the observation can be propagated with the model dynamics by forcing it directly in a in-stream simulation on a new state vector $y_k$. The physical system represented by $y_k$ should reflect the observation in the region where it is available. The other regions of this physical system are affected by the observation through model propagation. $y_k$ could be written as:
\begin{equation}
    y_k=\Phi_k y_{k-1}+K(z_k-y_k)\label{eq:z_prop}
\end{equation}
Equation \eqref{eq:z_prop} is reminiscent of the update equation for the KF estimate \eqref{eq:x_kf} but now the gain $K$ is considered to be equal to the unity matrix $I$. The error covariance matrix can be estimated as follows:

\begin{equation}
    P_{k}=\mathbb{E}[(\hat{x}_{k|k}-y_k)(\hat{x}_{k|k}-y_k)^T]\label{eq:P_kf_def_y}
\end{equation}

The error of the system is now estimated using $y_k$ which is a crude approximation of the true state of the system $x^{true}_k$. In conclusion, $y_k$ contains the physical meausrement information in the region defined by the observation window. This information is propagated with the state transition matrix to the other regions of the numerical domain. The information represented in $y_k$ is then compared to the \textit{a priori} estimation $x_{k|k-1}$ and $P_{k|k}$ is calculated.

The error covariance estimation can be applied to the multiple grid framework. To reduce the computation cost associated to the propagation of $z_k$, the state-transition model for $y_k$ can be constructed on a coarser grid with the conditions that the global dynamics of the system can be correctly captured on this grid. For convenience, we consider that in the following equations $y_k$ and $z_k$ share the same grid resolution. However, different meshing strategies can be used. The multiple grid KF algorithm with the in-stream estimation of the error covariance matrix can be conceptualized in a two-phase process:  

\begin{enumerate}
  \item A predictor phase, where $x_{k-1|k-1}$ is advanced through the state transition model $\Phi_k$ on the fine grid and an \textit{a priori} estimation is calculated. The observation is forced and propagated on $y_k$ and the error covariance matrix is estimated:
  \begin{eqnarray}
    &\hat{x}_{k|k-1}^F=\Phi_k^F\hat{x}_{k-1|k-1}^F\label{eq:x_mdl_kfmg_PE}\\
    &\hat{x}_{k+1|k}^C=\Pi^{F\rightarrow C}(\hat{x}_{k+1|k}^F)\label{eq:x_mdl_kfmg_PE_coarse}\\
    &y_{k}^C=\Phi_k^C y_{k-1}^C+(z_k^C-H^C_ky_{k-1}^C)\label{eq:y_md_kf}\\
    &P_{k|k}^C=(\hat{x}_{k|k-1}^C-y_{k}^C)(\hat{x}_{k|k-1}^C-y_{k}^C)^T\label{eq:P_mg_E}
  \end{eqnarray}
  \item An update phase, where observation is integrated through the Kalman Filter on the coarse grid.$y_k$ maps the flow characteristics not just on the observation window but everywhere else, allowing to construct error correlations between the observation window and the other regions of the numerical domain.
  \begin{eqnarray}
    &K_k^C=P_{k|k-1}^C{(H_k^C)}^T(H_k^C P_{k|k-1}^C {(H_k^C)}^T+R_k^C)^{-1}\label{eq:K_kfmg_PE}\\
    &\hat{x}_{k|k}^F=\hat{x}_{k|k-1}^F + \underbrace{\Pi^{C\rightarrow F}\big  (K_k^C(z_k^C-H_k^C\hat{x}_{k|k-1}^C)\big)}_\text{KF Correction}\label{eq:x_kfcmg_PE}
  \end{eqnarray}
\end{enumerate}

%Drawback of using diagonal Q (localized corrections where observation is available, no cross-correlation between the variables nor spatial correlation)
%Idea, how to prove that the estimation of P makes sense. Start a test with the true value and say that the uncertainties are coming from not knowing the exact boundary conditions. Then start a simulation with forcing the observation...

\section{Results: preliminar analyses for one-dimensional test cases}
The multiple-grid KF algorithm is tested on the viscous Burgers' 1D case described in equation \eqref{eq:burgers}. We study the temporal and spatial evolution of $u(x,t)\in\mathbb{R}^N$ as dictated by the Burgers' viscous model. The discretized form of the aforementioned equation can be represented as written in equation \eqref{eq:burgers_compact_discre_compact}. The discretization of time derivatives is performed using an explicit forward Euler scheme and a second-order centered scheme is used for the spatial derivatives. The initial state of the system is set at a constant value $u(x,0)=u_0$. The inlet boundary condition is perturbed with a time dependent sinusoidal forcing: $u(0,t)=u_0+\sum_{i=1}^{n} \epsilon_i (u_0\sin(w_i t))$, where $n$ is the number of modes used to force the inflow and $\epsilon_i$ and $\omega_i$ represent their respective relative forcing intensity and oscillation frequency. The outflow boundary conditition is defined using linear extrapolation. 

Two grid systems with the same length $L_x$ are constructed. On the first grid, a very fine resolution is set in order to finely capture the dynamics of the flow. Following the notation used in the previous sections, the flow on the fine grid at an discrete instant $k$ is defined as $u^F_k$. The second grid is coarser and the representation of the flow at an instant $k$ is defined as $u^C_k$. A twin-experiment is conducted where:
\begin{enumerate}
\item Given an initial condition $u^F_0$, the flow is propagated on the fine grid with the model dynamics $\Phi_k^F$, to a state $u^F_K$ as described in equation \eqref{eq:burgers_compact_discre_compact}. The representation of $u$ from $0\leq k \leq K$ is considered to be the \textit{True} discrete state of the system (the model is assumed exact).
\item For each calculated time-step, $u^C_k$ is obtained as a projection of $u^F_k$ on the coarse grid:
\begin{equation}
u^C_k=\Pi^{F\rightarrow C}(u^F_k)\label{eq:u_fProju_c}
\end{equation}
where $\Pi$ is a projection operator. In this study it represents a centered five-point interpolation process (Lagrange Polynomial). An observation database is built by adding artificial gaussian noise to $u_k^C$:
\begin{equation}
z^C_k=u^C_k+v_k\label{eq:obser_const}
\end{equation}
where $v_k \sim \mathcal{N}(0,R)$ and R represents the error variance.
\item A new data-drive simulation on the fine grid is started with the same initial condition $u^F_0$, but the inflow is no longer perturbed $u(0,t)=u_0$. The noisy observation data $z^C$ is integrated through the multiple-grid KF. The accuracy of the filtering process is analysed by comparing the results to the \textit{True} state of the flow.
\end{enumerate} 

\subsection{Multiple-KF Twin Experiment : one perturbation mode}
A first test is performed where total number of inlet perturbation modes is set to $n=1$. The length of the domain is defined as $L_x=10\lambda$, where $\lambda$ is the wavelength of the sinusoidal inlet forcing. The forcing intensity $\epsilon$ is set to 1$\%$, in order to have a quasi-linear evolution of the inlet perturbations. The total simulation time is $K=3t_c$, where $t_c=L_x/u_0$ represents the characteristic advection time of the system. The total number of elements in the fine grid $N_F$ is set to 800 in order to have a resolution of 80 points per wavelength on the fine grid. The resolution of the coarse grid is set to 20 points per wavelength. The CFL number ($u_0 \Delta t/\Delta x$) of the \textit{True} simulation is set to 0.02. The observation database is constructed as described before. $z_k^C$ is a random gaussian variable characterized by a mean value corresponding to the true projected value on the coarse grid and a standard deviation of $\sigma=0.05u_0$, thereby $z_k^C\sim\mathcal{N}(u_k^C,\sigma^2)$. In Fig.\ref{fig:true_noise}, the \textit{True} state of the flow is represented along with the artificially created observation $z$.
\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\textwidth]{true_noise.png}
\caption{\label{fig:true_noise}Snap of the \textit{True} state of the system and the noisy observation $z$ for a total \textit{True} simulation time $t_T=1.01t_c$. The grey area from $[0\leq x \leq 1]$ depicts the actual zone where observation is available.}
\end{figure} 

The data-driven simulation is started with the same numerical configuration described for the \textit{true} simulation but, without inflow forcing. In the following, we adopt the notations used in the definition of the multiple-grid KF algorithm. We assume that the observation data are not available at every instant $k$. We consider that $z^C_k$ is available every 30$\Delta t$, which amounts to roughly 120 assimilation cycles per $\lambda$. The first observation integrated to the data-driven simulation $z^C_0$ at $t_S=0$, corresponds to the \textit{True} state at an instant $t_T=1$, where time is adimensioanlized by the characteristic advection time. We assumed that the available observation is limited to an observation window defined as $[0\leq x\leq 1]$, where the length $x$ is adimensionalized with $\lambda$.

No prior knowledge is assumed about the error covariance matrix, therefore it is initialized as $P^C_{0|0}=0$. The measurement error covariance matrix $R^C_k$ is considered to be diagonal and constant in time $R^C=\sigma^2$. In this first test, the state-transition operator $\Phi^F_k$ is considered exact. Nonetheless, the inflow boundary conditions provided in this second, data-driven calculation differ from the ones of the \textit{True} simulation and the results obtained diverge considerably. The challenge in this context is to provide an accurate model error covariance matrix $Q^C_k$ that characterizes the bias due to the boundary conditions uncertainties. Different authors [REF] propose a diagonal $Q_k$ proportional to $cI$, where $I$ is the identity matrix and $c$ is a coefficient analogous to the variance of the observation $\sigma^2$. It is interesting to analyse the influence of the prescribed model error variance $c$ in the assimilation process. If $Q^C_k$ and $R^C_k$ represent diagonal, constant in time matrices and the error covariance matrix is fixed \eqref{eq:P_kfmg_fixed}, it can be proven that $P^C_{k|k}$ reaches a quasi-steady state. Due to the diagonal form of the error covariance matrices we can directly write:
\begin{equation}
K_k^C=\frac{P^C_{k|k-1}+Q^C}{P^C_{k|k-1}+Q^C+R^C}\label{eq:Kalman_Gain_diagonal}
\end{equation}
It follows that the Kalman Gain $K^C_k$ also reaches a quasi-steady state and it entirely depends on $c$ ($Q_k^C=c I$) and $\sigma$, which is fixed for this case. An analysis of the influence of $c$ is therefore presented for different values of $K^C_k$ $[0\leq K_k^C \leq 1]$, where zero represents an infinite confidence in the model prediction ($c<<\sigma^2)$ and one represents an infinite confidence in the observation ($c>>\sigma^2$). Remember that the Kalman Gain is the relative weight given to the observation or the model prediction. The synchronization of the data-driven simulation with the \textit{True} state of the system is tracked with the integrated RMSE across the entire domain for each instant k and an averaged RMSE over the total assimilation time:
\begin{eqnarray}
	&RMSE_k=\sqrt{\sum_{i=1}^{N_f}\frac{(x^{True}_{k_i}-x^F_{{k|k}_i})^2}{N_f}}\label{eq:RMSE_k}\\
	&\overline{RMSE}=\frac{1}{K}\int^K_0\sqrt{\sum_{i=1}^{N_f}\frac{(x^{True}_{k_i}-x^F_{{k|k}_i})^2}{N_f}}dt\label{eq:RMSE_avg}
\end{eqnarray}

In Fig. \ref{fig:Kanalysis} we present the RMSE of the multiple-grid KF estimator for different Kalman Gain coefficients.
\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\textwidth]{Kanalysis.png}
\caption{\label{fig:Kanalysis}Performance of the estimator in terms of the Root Mean Square Error (RMSE) for an assimilation window of two characteristic advection times. A parametric study is performed to analyse the influence of the Kalman Gain. The blue color line represents the performance of the estimator when the exact error covariance matrix is provided.}
\end{figure}
The best results are obtained when the prescribed error covariance matrix is exact (it is possible to do so in this case as the true state of the system is available), and we used this case to monitor the relative  performance of the estimator. As expected, the reconstruction of the flow is complete and instantaneous if the \textit{True} error covariance matrix is provided. In the other cases, the synchronization process is gradual. Nonetheless, this is expected as the observation data is integrated very close to the inlet and the information is propagated downstream by the state-transition operator $\Phi^F_k$. We observe that for all the cases, the RMSE over the domain is gradually reduced until the information reaches the outflow boundary of the domain, a process which requires an advection time to be completed ($t_c$). Thereafter, the measured RMSE is stabilized.

To asses the overall performance of the estimator, we present in Fig. \ref{fig:Kanalysisaverage} the $\overline{RMSE}$ for the assimilation processes in function of the Kalman Gain.
\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\textwidth]{Kanalysisaverage.png}
\caption{\label{fig:Kanalysisaverage}Performance of the estimator in terms of the integrated RMSE over the entire assimilation window.}
\end{figure}
It is interesting to observe that three clear operating regimes emerge:
\begin{enumerate}
\item \textbf{Optimal Regime}. There exists an optimal steady-state Kalman Gain which minimizes the RMSE and thereby, assures the synchronization of the twin-experiment. As the measurement error variance $\sigma^2$ is fixed, the estimator is completely controlled by the error model variance coefficient $c$. The results show that for this test-case, the minimum RMSE is found when the relative confidence in the model is greater than the one given to the measurements ($\sigma^2 > c$). The actual minimum point ($K^C= 0.06$ in this case) is dictated by the noise in the measurement $\sigma$ and especially, by the frequency of the available data (120 observations per $\lambda$ in this case). The minimum RMSE point should shift to the left of the curve with a higher frequency (more confidence in the model error) and to the right with a lower frequency (less confidence in the model). In terms of absolute performance, we expect the accuracy of the estimator to weaken with sparser (in time) observation. In Fig.\ref{fig:optimalK} we present a snap of the estimator $x^F_{k|k}$ for a total simulation time of $t_S =1.15$.
\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\textwidth]{optimalK.png}
\caption{\label{fig:optimalK}Snap of the estimator $x_{k|k}^F$ for $K^C=0.06$ and the \textit{True} state of the system for a total simulation time of $t_S=1.15$. The red line represents the KF Correction. The grey area from $[0\leq x \leq 1]$ depicts the actual zone where observation is available.}
\end{figure}
\item \textbf{Underprediction of the model error variance $c$.} When the model error variance is underpredicted we observe a very rapid decline in the performance of the estimator. In Fig.\ref{fig:underpredK} we present a snap of the estimator for $K^C=0.005$, an extreme case of underprediction. 
\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\textwidth]{underpredictedK.png}
\caption{\label{fig:underpredK}Snap of the estimator $x_{k|k}^F$ for $K^C=0.005$ and the \textit{True} state of the system for a total simulation time of $t_S=1.15$. The red line represents the KF Correction. The grey area from $[0\leq x \leq 1]$ depicts the actual zone where observation is available.}
\end{figure}
It is interesting to notice that the signal, although in perfect phase with the \textit{True} state, is underpredicted. Since the confidence in the model is too high, the relative weight given to the observation is too small to allow the complete resynchronization of the twin-flow experiment. In conclusion, if the model error covariance matrix is underpredicted, the estimation is underpredicted but smooth.
\item \textbf{Overprediction of the model error variance $c$.}  In this operating regime, the relative weight given to the measurement is too high and the performance of the estimator is diminished. However, the loss of performance is of different nature in this case and not due to underprediction.  If the relative weight of the observations in the KF process is overpredicted, the noise present in this observations may disrupt the estimate. In extreme cases it might even affect the numerical stability of the simulation if high gradients exist. In Fig. \ref{fig:overpredK} we present a snap of the estimate for $K^C=0.80$:
\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\textwidth]{overpredK.png}
\caption{\label{fig:overpredK}Snap of the estimator $x_{k|k}^F$ for $K^C=0.80$ and the \textit{True} state of the system for a total simulation time of $t_S=1.15$. The red line represents the KF Correction. The grey area from $[0\leq x \leq 1]$ depicts the actual zone where observation is available.}
\end{figure}
Notice that the high-frequency components of the observation are integrated into the model and propagated downstream through the dynamical system. Therefore, the performance of the estimator is significantly affected. 
\end{enumerate}
In conclusion, we have tested the multiple-grid KF estimator on a one-dimensional test-case with promising performance results. The limitations of the methodology used are also clear. Since we assume diagonal error covariance matrices and the propagation of the error statistics is fixed, the estimator modifies the flow only on the region where observation is present. A second drawback of the algorithm is that it depends significantly on the model error covariance matrix, which is not known a priori. Nonetheless, the twin-experiment presented in this section permits to draw important conclusions. As Evensen et al state in [REF annual review geo 2018], the model is paramount. The overall confidence given to the model should be higher than the one given to the measurements. The smoothness of the final solution is also an important factor to be monitored in the estimator. In a practical case, a convergence analysis could be performed where the control parameter is the prescribed model error variance $c$. However, the overall performance of the estimator depends significantly on the frequency of the available measurements. A smooth estimate does not inherently imply an accurate result since underprediction might still be present. 

==> out <==
additionalMaterialByGabriel.tex:    \item The grid resolutions used in the compressible flow simulation framework are often extremely fine, which is necessary to capture the complete dynamics of the physical system. However, the type of mesh resolutions attainable through experimental measurement, such as Particle Image Velocimetry (PIV) for example, is orders of magnitude lower [REF]. In addition, the large coherent flow structures captured through direct measurement, which dictate the global dynamics of the flow [REF and some more information, maybe interesting], are sufficiently well defined with coarser resolutions. In conclusion, there are strong arguments for the application of the KF algorithm in a multiple grid framework where the state transition calculations are performed in a fine grid and the statistical modifications of the flow are performed in a secondary coarser grid. [ADD a FIGURE MAYBE]
additionalMaterialByGabriel.tex:Let us define two spaces or grids that describe the same physical phenomena $x_k$ at an instant $k$. Let $x_k$ on the first space be defined as $x_k^F$, where $F$ stands for the representation of the phenomena on the fine grid. Consider that the current time-step of the phenomena has been calculated from a previous instant $k-1$ with the state-transition model. Let $x_k$ on the second space be defined as a projection of the fine grid representation on the coarse grid $x_k^C=\Pi^{F\rightarrow C}(x_k^F)$, where $\Pi$ is a projection operator. Consider now that observation $z_k^C$ at an instant $k$ is available on a coarse grid and the KF is to be applied in order to correct the representation of the phenomena on the fine space $x^F_k$. Considering the hypothesis discussed in the previous paragraph, the framework now presented allows for the application of the KF on the coarse grid, where $x_k^C$ and $z_k^C$ are integrated and a KF estimate $\hat{x}_k$ is obtained. In practice, the developed Multiple Grid KF algorithm can be conceptualized as a two-phase process:
additionalMaterialByGabriel.tex:Note that the superscripts $F$ and $C$ indicate if the variable which they accompany is represented on the fine or the coarse grid, respectively. It is straightforward to recognize the canon form of the KF in the Multiple Grid KF algorithm that we present. The major difference is that the KF correction is calculated not on the same space as where the state-transition is performed, but on a projection of a coarser version of this space. The coarse KF correction is then projected back on the fine space.
additionalMaterialByGabriel.tex:The forecast error covariance matrix $(P^e)^C_{k|k-1}$ is transferred every instant there is an observation to the first  sub-process, where the fine grid simulation is corrected with the error statistics calculated in the ensemble sub-process. If the analysis error covariance $(P^e)^C_{k|k}$ is required, it can be obtained from the ensemble, but it is not necessary for the algorithm to perform, as the error statistics are correctly characterized in the ensemble. 
additionalMaterialByGabriel.tex:$P_{k|k}$, or the error covariance matrix describes the probabilistic behavior of the error in the KF estimate $\hat{x}_{k|k}$. Assuming that both observation and model error can be described by Gaussian PDF it follows that the KF estimate $\hat{x}_{k|k}$ is a Gaussian process $\hat{x}_{k|k}\sim \mathcal{N}(x^{true}_k,P_{k|k})$ and $\hat{e}_{k|k}\sim \mathcal{N}(0,P_{k|k})$. The diagonal elements of $P_{k|k}$ represent the error variance of each element in the vector state estimate $\hat{x}_{k|k}$ and the off-diagonal terms describe the covariance of each pair of components in $\hat{x}_{k|k}$. The error covariance is of pivotal importance. It describes the error correlations in the system and is responsible for the transferring of information between the multiple components of the state vector. For example, in the framework of sequential data assimilation, an accurate and complete $P_{k|k}$ would allow the KF algorithm to correct variables that are not directly observed. The error correlations present in $P_{k|k}$ influence the calculation of the Kalman Gain, which in turn dictates how each observed component of the state vector is corrected and how they affect the correction of their zone of influence.
additionalMaterialByGabriel.tex:The error of the system is now estimated using $y_k$ which is a crude approximation of the true state of the system $x^{true}_k$. In conclusion, $y_k$ contains the physical meausrement information in the region defined by the observation window. This information is propagated with the state transition matrix to the other regions of the numerical domain. The information represented in $y_k$ is then compared to the \textit{a priori} estimation $x_{k|k-1}$ and $P_{k|k}$ is calculated.
additionalMaterialByGabriel.tex:  \item A predictor phase, where $x_{k-1|k-1}$ is advanced through the state transition model $\Phi_k$ on the fine grid and an \textit{a priori} estimation is calculated. The observation is forced and propagated on $y_k$ and the error covariance matrix is estimated:
additionalMaterialByGabriel.tex:\item For each calculated time-step, $u^C_k$ is obtained as a projection of $u^F_k$ on the coarse grid:
additionalMaterialByGabriel.tex:No prior knowledge is assumed about the error covariance matrix, therefore it is initialized as $P^C_{0|0}=0$. The measurement error covariance matrix $R^C_k$ is considered to be diagonal and constant in time $R^C=\sigma^2$. In this first test, the state-transition operator $\Phi^F_k$ is considered exact. Nonetheless, the inflow boundary conditions provided in this second, data-driven calculation differ from the ones of the \textit{True} simulation and the results obtained diverge considerably. The challenge in this context is to provide an accurate model error covariance matrix $Q^C_k$ that characterizes the bias due to the boundary conditions uncertainties. Different authors [REF] propose a diagonal $Q_k$ proportional to $cI$, where $I$ is the identity matrix and $c$ is a coefficient analogous to the variance of the observation $\sigma^2$. It is interesting to analyse the influence of the prescribed model error variance $c$ in the assimilation process. If $Q^C_k$ and $R^C_k$ represent diagonal, constant in time matrices and the error covariance matrix is fixed \eqref{eq:P_kfmg_fixed}, it can be proven that $P^C_{k|k}$ reaches a quasi-steady state. Due to the diagonal form of the error covariance matrices we can directly write:
App1.tex:\caption{\label{fig:2D-mxl-trutht11}Flow calculated using a 2D Navier-Stokes equation. Visualization of the normal velocity field for the reference simulation for $t=11t_c$.}
App1.tex:  \caption{\label{fig:MGENKF_states_rc4} Time evolution of the quantity $\rho v$ at the centerline of the mixing layer, calculated using the Multigrid EnKF (MEnKF) estimator. The case for $r_C=4$ is here shown. Total simulation time of $t=1$, $t=5$ and $t=33$ (in $t_c$ units) for state (a), (b) and (c), respectively. The blue line represents the True state, the orange line is the estimator and the red line is the EnKF correction. }
App1.tex:  \caption{\label{fig:MGENKF_states_rc4} Time evolution of the quantity $\rho v$ at the centerline of the mixing layer, calculated using the Multigrid EnKF (MEnKF) estimator. The case for $r_C=4$ is here shown. Total simulation time of $t=1$, $t=5$ and $t=33$ (in $t_c$ units) for state (a), (b) and (c), respectively. The blue line represents the True state, the orange line is the estimator and the red line is the EnKF correction. }
App2_Moldovan.tex:%      Calculation of statistics from the coarse state ensemble: $\overline{x}_k^{f,C}=\frac{1}{N}\sum_{n=1}^{N}x_k^{f,C,(i)} $; $X_k^C=\frac{1}{\sqrt{N-1}}\big[x_k^{f,C,(1)}-\overline{x}_k^{f,C},...,x_k^{f,C,(N)}-\overline{x}_k^{f,C}\big]$ \\
App2_Moldovan.tex:%      Calculation of statistics from the parameter ensemble:
App2_Moldovan.tex:%      Kalman Gain Calculation: $K_k^{e,C}=X_k^C Y^T(Y Y^T+R^C)^{-1}$; $K^{e,C,\theta}_k=\Theta_k Y^T(Y Y^T+R^C)^{-1}$; $Y=\mathcal{H}^C X_k^C$ \\
App2_Moldovan.tex:%      Calculation of statistics from the coarse state ensemble: $\big(\overline{x}_k^{f}\big)^C=\frac{1}{N}\sum_{n=1}^{N}\big(x_k^{f,(i)}\big)^C $; $\big(X^f_k\big)^C=\frac{1}{\sqrt{N-1}}\Big[\big(x_k^{f,(1)}\big)^C-\big(\overline{x}_k^{f}\big)^C,...,\big(x_k^{f,(N)}\big)^C-\big(\overline{x}_k^{f}\big)^C\Big]$ \\
App2_Moldovan.tex:%      Calculation of statistics from the parameter ensemble:
App2_Moldovan.tex:%      Kalman Gain Calculation: $\big(K_k^{x,e}\big)^C=\big(X_k^f\big)^C Y_k^T(Y_k Y_k^T+R_k^C)^{-1}$; $\big(K^{\theta,e}_k\big)^C=\Theta^f_k Y_k^T(Y_k Y_k^T+R_k^C)^{-1}$; $Y_k=\mathcal{H}_k^C \big(X^f_k\big)^C$ \\
App2_Moldovan.tex:%\item In the conceptual algorithm, $\left(x^{C}_k\right)^{'}$, is calculated iteratively by time-integrating $\left(x^{C}_k\right)^{*}$ with an implicit scheme. Assuming small $\Delta t$, $\left(x^{C}_k\right)^{'}$ can be directly calculated in a Kalman Filter fashion:$\left(x^{C}_k\right)^{'}=\left(x^{C}_k\right)^{*}+\left(K_k^C\right)^{x,e}\left[\left(y_k^{C}\right)^o-\mathcal{H}_k^C\left(\left(x_k^{C}\right)^{*}\right)\right]$. Note that by doing this the correction on the fine grid is not necessarily constrained and the smoothness of the solution will depend on the quality of the Kalman Gain operator $\left(K_k^C\right)^{x,e}$. 
Main_Cordier.tex:\newcommand{\todolc}[1]{\textbf{\textcolor{red}{TODOLC: #1}}}
Main_Cordier.tex:\newcommand{\lc}[1]{\textbf{\textcolor{green}{LC: #1}}}
Main_Cordier_Gabriel_ver.tex:\newcommand{\todolc}[1]{\textbf{\textcolor{red}{TODOLC: #1}}}
Main_Cordier_Gabriel_ver.tex:\newcommand{\lc}[1]{\textbf{\textcolor{green}{LC: #1}}}
Main_Moldovan.tex:\newcommand{\lc}[1]{\textbf{\textcolor{green}{LC: #1}}}
Sec0.tex:\todo{Le fil conducteur du papier n'est pas clair à suivre. On a l'impression que tous les mots-clés ont été mis dans le titre : "intrusive", "multigrid" et "ensemble" (name dropping). Le caractère "intrusive" ou non doit être commenté. Ne serait-ce pas d'ailleurs "non intrusive" ! Je ne vois pas le caractère "intrusive" comme un avantage. Au niveau de l'organisation du papier, j'aurais envie de commencer par la description de KF, d'expliquer les limites dues au problème de grande taille puis d'introduire le multigrille comme un moyen d'économiser du temps de calcul. }
Sec0.tex:\lc{Si je ne me trompe pas, nous sommes passés dans les développements numériques d'une approche où le coeur était l'utilisation d'une stratégie multigrille (à deux grilles en l'occurence) pour KF à une stratégie reposant sur l'EnKF et sur l'utilisation des deux grilles. EnKF est déjà considéré dans la communauté DA comme une méthode permettant de réduire le coût de calcul en estimant la matrice de covariance via une méthode d'ensemble plutôt qu'en la transportant. Il faudrait donc a prori tester cette méthode sur une même grille et montrer quel est le nombre d'individu minimum qu'il faut considérer pour obtenir une bonne représentation de la matrice de covariance. Cela nous donnerait alors un cas de référence à partir duquel on pourrait envisager des comparaisons. La stratégie à deux grilles ne serait alors là que pour montrer que le coût de calcul est réduit ou qu'à un coût de calcul donné l'erreur d'estimation est la même. Est-ce là l'objectif ?}
Sec0.tex:\lc{Nous avons besoin (j'ai besoin) d'avoir une description claire et nette des tests numériques que Gabriel réalise. Gabriel a obtenu beaucoup de résultats mais il est souvent difficile de savoir dans quelles conditions les tests ont été réalisés. du coup, il est difficil en l'état de connecter les sections "méthode" des sections "application". Imaginons que nous nous concentrons d'abord sur une équation de Burgers comme dans la section 4. Quel est alors l'objectif de l'assimilation de données ? Coment l'équation de Burgers a été résolu. Tout cela doit être précisé.} 
Sec1.tex:Data Assimilation (DA) \cite{Asch2016_SIAM,Evensen2009_Springer,Daley1991_cambridge} for weather prediction, ocean modelling and more recently  mechanical engineering problems. Essentially, DA methods combine information issued from two sources: i) a \emph{model}, which provides a dynamical description of the phenomenon in the physical domain, ii) a set of \emph{observations}, which are usually sparse and/or local in time and space.  These methods are classified  in different families according to the way the state estimation is performed. One of the classical criterion of classification deals with the operative strategy used to derive the state estimation. \emph{Variational} approaches resolve a constrained optimization problem over the parametric space characterizing the model (usually coefficients defining boundary conditions or physical models). The solution of the variational problem minimizes prescribed error norms so that the assimilated model complies with the observation provided over a specified time window. Methods from this family, which include $3$D-Var and $4$D-Var, usually exhibit very high accuracy \cite{Onder2016_cf,Foures2014_jfm,Mons2019_jcp,Chandramouli_Memin_Heitz_JCP_2020}. However, they are also affected by several drawbacks. First, the formulation of the adjoint problem that is introduced to perform the parametric optimization can be difficult, if not impossible, when automatic differentiation is not employed. Second, the adjoint problem is defined backward in time which may lead to numerical difficulties of resolution related to  the unaffordable data storage that is needed, and the amplification of the adjoint solution that frequently happens when multi-scale interactions are dominant \cite{Asch2016_SIAM,Onder2016_cf,Sirkes1997_mwr}. Third, standard variational data assimilation methods are \emph{intrusive} from a computational point of view, requiring the development of an adjoint calculation code, or the availability of the source code  when the use of automatic differentiation is planned.  In most cases, modifications are required in order to maintain the code or extend the applications (change of the definitions of errors, for instance). For commercial software without open-source licence, these modifications are expensive. \emph{Non-intrusive} methods that require no modification of original calculation code are therefore preferable in data assimilation. 
Sec1.tex:Another family of DA methods is represented by the \emph{sequential} approaches. These methods, mostly based on Bayes' theorem, provide a probabilistic description of the state estimation. A well known approach is the Kalman Filter (KF) \cite{Kalman1960_jbe}. Extensions and generalizations of this method have also been developed, such that the Extended Kalman Filter (EKF) \cite{Welch_Bishop_Report_2006} which is tailored for nonlinear systems, and Ensemble Kalman Filter (EnKF) \cite{Evensen2009_Springer}. This class of methods solves the state estimation problem by transporting error covariance matrices of the model and observations. These methods are usually more flexible than variational approaches (no required computation of first order sensitivities), but the time advancement and update of the covariance matrices are prohibitively expensive for large scale problems, encountered in practical applications \cite{Rozier_Birol_Cosme_Brasseur_Brankart_Verron_SIAM_Review_2007}. One possible strategy consists in reducing the order of the Kalman filter \cite{Suzuki2012_jfm} or filtering the error covariance matrix. Inspired by a domain localization procedure, Meldi \& Poux \cite{Meldi2017_jcp,Meldi2018_ftc} proposed  a strategy based on an explicit filter of the error covariance matrix. The application of this estimator to different turbulent flows exhibited encouraging results considering the relatively small increase in computational resources. A more popular strategy for data assimilation of engineering applications is the Ensemble Kalman Filter \cite{Asch2016_SIAM,Evensen2009_Springer,Evensen2009_IEEE}, which relies on a Monte Carlo implementation of the Bayesian update problem. The EnKF (and follow-up models) was introduced as an extension of the original Kalman filter made for high-dimensional systems for which transporting the covariance matrix is not computationally feasible. EnKF replaces the covariance matrix by the sample covariance matrix computed from an ensemble of state vectors. The main advantage of EnKF is that advancing a high-dimensional covariance matrix is achieved by simply advancing  each member of the ensemble.  Several research works have been reported in the literature in recent years for application in fluid mechanics \cite{Mons2016_jcp,Xiao2016_jcp,Rochoux2014_nhess}. Despite the interest of this non-intrusive technique, and the possibility to perform efficient parametric inference, the computational costs can still be prohibitive for realistic applications. Statistical convergence is usually obtained for a typical ensemble size going from $60$ to $100$ ensemble members \cite{Asch2016_SIAM}.         
Sec1.tex:In addition, the state estimation obtained via sequential tools does not necessarily comply with a model solution i.e. the \textit{conservativity} of the dynamic equations of the model is violated. This aspect is a potentially critical issue in fluid mechanics studies. Violation of conservativity may result in loss of conservation of some physical properties of the flow (such as mass conservation or momentum conservation) as well as in the emergence of non-physical discontinuities in the flow quantities. The aforementioned issues significantly affect the precision of the prediction of the flow and may eventually produce irreversible instabilities in the time advancement of the dynamical model. A number of works in the literature have provided advancement in the form of additional constraints to be included in the state estimation process. Meldi \& Poux \cite{Meldi2017_jcp} used a recursive procedure and a Lagrangian multiplier (the pressure field) to impose the zero-divergence condition of the velocity field for incompressible flows. Other proposals deal with imposing hard constraints in the framework of an optimization problem \cite{Simon2002_IEEE}, ad-hoc augmented observation \cite{Nachi2007_IEEE} and generalized regularization \cite{Zhang2020_jcp}. These approaches are responsible for a significant increase in the computational resources required, which is due to augmentation in size of the state estimation problem or to the optimization process, which usually needs the calculation of gradients of a cost function.        
Sec1.tex:Multigrid methods \cite{Brandt1977_mc,Ferziger2002_springer} are a family of tools which employ multi-level techniques to obtain the time-advancement of the flow. In particular, the geometric multigrid \cite{Wesseling1999_jcam} uses different levels of the resolution in the computational grid to obtain the final state. The method here proposed exploits algorithmic features of iterative solvers used in practical CFD applications. The EnKF error covariance matrix reconstruction is performed using information from a number of ensemble members which are generated over a coarse level mesh of a multigrid approach. This procedure is reminiscent of reduced order / multilevel applications of EnKF strategy reported in the literature \cite{Hoel2016_SIAM,Siripatana2019_cg,Fossum2020_cg,Brajard2020_arxiv}. However, the state estimation obtained at the coarse level is used to obtain a single solution calculated on a high resolution mesh grid, similarly to the work by Debreu et al. \cite{Debreu2015_qjrms} for variational DA. Because of the algorithmic structure of the problem, all of the simulations on the fine and coarse level can be run simultaneously in parallel calculations, providing a tool able to perform in-streaming DA for unsteady flow problems.
Sec1.tex:%\lc{à revoir à la fin} 
Sec2.tex:The classical KF algorithm is not suited for direct application to the analysis of complex flows. First of all, KF classical formulation is developed for linear systems. Applications to non-linear systems can be performed using more advanced techniques such as the extended Kalman filter \cite{Welch_Bishop_Report_2006} or exploiting features of the numerical algorithms used for numerical discretization \cite{Meldi2017_jcp}.
Sec2.tex:\item Starting from an initial solution on the fine grid $\left(\mathbf{x}^0\right)^\text{\tiny F}$ (which is usually equal to $\mathbf{x}$ at the previous time step $k-1$), an iterative procedure is applied to obtain a first solution $\left(\mathbf{x}^1\right)^\text{\tiny F}$. A residual $\left(\mathbf{\delta}^1\right)^\text{\tiny F}= \mathbf{c}^\text{\tiny F} - \mathbf{\Psi}^\text{\tiny F} \left(\mathbf{x}^1\right)^\text{\tiny F}$ is calculated.
Sec2.tex:$\left(\mathbf{x}^3\right)^\text{\tiny F}$. Performing part of the calculations on a coarse grid level provides two main advantages \cite{Ferziger2002_springer}. First, a significant reduction in the computational resources is obtained
Sec2.tex:since the calculations performed over the coarse grid are usually much less expensive than a full set of iterations over the fine grid.
Sec3.tex:\item[-] As previously stated, $\mathbf{\Psi}^\text{\tiny C}$ and its role in the determination of the matrices $\left(\mathbf{\Psi}^\text{\tiny C}\right)^{(i)}$ is an essential step in the MEnKF strategy. In non-linear problems of interest in fluid mechanics, the state transition matrix $\mathbf{\Psi}$ includes information of the multi-scale interactions that are specific for every case investigated. The simplest possible choice, which is the one adopted in this work, is to calculate the coefficients of the matrices $\mathbf{\Psi}^\text{\tiny C}$ and $\left(\mathbf{\Psi}^\text{\tiny C}\right)^{(i)}$ separately for each simulated state. Thus, the similarities between the employed state matrices are limited to the use of the same discretization schemes / structure of $\mathbf{\Psi}$. However, one can envision to use the non-linear information conserved in $\mathbf{\Psi}^\text{\tiny C}$, which is supposedly accurate, to improve the accuracy of the prediction of the ensemble members. This aspect is discussed in the perspectives included in Sec.~\ref{sec:conclusions}.
Sec3_2020_11_16_12_52.tex:The multigrid-ensemble algorithm works through the steps described below. In the following description, $\mathbf{\Psi}$ might hold for both $\mathbf{\Psi}$ and/or $\widetilde{\mathbf{\Psi}}$ described in equation \eqref{eq:generalDiscretizedFormInt}, depending on the choice of the time integration strategy. Note that the states $\left(\mathbf{x}^\text{C}_{k}\right)^{*}$ and $\left(\mathbf{x}^\text{C}_k\right)^{'}$ are associated to the single fine-grid simulation only and are natural to the FAS multigrid method described before. They represented the projection on the coarse-grid of the first fine-grid solution ($\left(\mathbf{x}^1\right)^\text{C}$ in the FAS algorithm) and the coarse-grid solution obtained with an iterative process starting from the first fine-grid solution projected on the coarse grid ($\left(\mathbf{x}^2\right)^\text{C}$ in the FAS algorithm), respectively. $\left(\mathbf{x}^\text{C}_k\right)^\text{e}$ represents an intermediary estimated-state used to calculate $\left(\mathbf{x}^\text{C}_k\right)^{'}$.  
Sec3_2020_11_16_12_52.tex:\item \textbf{First iteration on the fine grid}. Starting from an initial solution on the fine grid $\left(\mathbf{x}^\text{F}_{k-1}\right)^\text{a}$, an iterative procedure is applied to obtain a forecast state $\left(\mathbf{x}^\text{F}_{k}\right)^\text{f}$. A residual $\mathbf{\delta}^\text{F}$ is calculated.
Sec3_2020_11_16_12_52.tex:\item \textbf{Time advancement of the ensemble members}. $\mathbf{\Psi}^\text{C}$ is used to determine the state matrices $\left(\mathbf{\Psi}\right)^{\text{C},(i)}$ \lc{je ne vois pas de quoi tu parles} for the advancement in time of the $N_\text{e}$ ensemble members defined on the coarse grid. The ensemble forecast $\left(\mathbf{x}^\text{C}_{k}\right)^{\text{f},(i)}$ is corrected with the standard EnKF procedure to obtain $\left(\mathbf{x}^\text{C}_{k}\right)^{\text{a},(i)}$. Also, the state estimation $\left(\overline{\mathbf{x}}^\text{C}_k\right)^\text{a}$ \lc{de quoi tu parles ?} and the parametric optimization are here performed.
Sec3_2020_11_16_12_52.tex:\item \textbf{Determination of the state variables on the coarse grid}. If observations are not available, the state $\left(\mathbf{x}^\text{C}_k\right)^{'}$  \lc{de quoi tu parles ?} ($\left(\mathbf{x}^2\right)^\text{C}$ in the FAS algorithm) is obtained using the classical multigrid procedure. On the other hand, if observations are available, the ensemble error covariance matrix $\left(\mathbf{P}_k^\text{C}\right)^{\text{f},\text{e}}$
Sec3_2020_11_16_12_52.tex: is used to determine the state estimation $\left(\mathbf{x}^\text{C}_k\right)^\text{e}$ \lc{de quoi tu parles ?}. The state estimation is used as initial condition in the coarse-grid iterative process in order to obtain $\left(\mathbf{x}^\text{C}_k\right)^{'}$ \lc{de quoi tu parles ?}. $\left(\mathbf{x}^\text{F}_k\right)^{'}$ \lc{de quoi tu parles ?} is then updated using the results obtained on the coarse space: $\left(\mathbf{x}^\text{F}_k\right)^{'}=\left(\mathbf{x}^\text{F}_{k}\right)^\text{f}+\Pi_\text{F}\left(\left(\mathbf{x}^\text{C}_k\right)^{'}-\left(\mathbf{x}^\text{C}_{k}\right)^{*}\right)$.
Sec3_2020_11_16_12_52.tex:Two different levels of representation (fine and coarse grids) are used to obtain a data-driven fine grid estimation.\todolc{Changer la notation des projecteurs.}\lc{je ne comprends pas cette figure}}
Sec3_2020_11_16_12_52.tex:\item[-] As previously stated, $\mathbf{\Psi}^\text{C}$ and its role in the determination of the matrices $\left(\mathbf{\Psi}\right)^{\text{C},(i)}$ is an essential step in the MEnKF strategy. In non-linear problems of interest in fluid mechanics, the state transition model $\mathbf{\Psi}$ includes information of the multi-scale interactions that are specific for every case investigated. The simplest possible choice, which is the one adopted in this work, is to calculate the coefficients of the matrices $\mathbf{\Psi}^\text{C}$ and $\left(\mathbf{\Psi}\right)^{\text{C},(i)}$ separately for each simulated state. Thus, the similarities between the employed state matrices are limited to the use of the same discretization schemes / structure of $\mathbf{\Psi}$. However, one can envision to use the non-linear information conserved in $\mathbf{\Psi}^\text{C}$, which is supposedly accurate, to improve the accuracy of the prediction of the ensemble members. This aspect is discussed in the perspectives included in Sec.~\ref{sec:conclusions}.
Sec3_2020_11_16_12_52.tex:However, these corrections may result in an increase of the computational resources required. Here, the multigrid algorithm itself is used for regularization (i.e. smoothing the discontinuities in the physical variables produced by the update via Kalman Filter) \lc{dans quel sens ?} of the flow. In fact, if an intentionally reduced tolerance is imposed in the iterative steps $4$ and $5$, the final solution will keep memory of the features of the state estimation produced in step $3$. However, the iterative resolution will smooth the estimation via the state transition model $\mathbf{\Psi}$, which will perform a natural regularization \lc{dans quel sens ?} of the flow. Clearly, if a reduced tolerance is imposed, the final solution will not necessarily respect the conservativity constraints of the model equations. However, one can argue that complete conservativity is not an optimal objective in this case, if the model state at the beginning of the time step is not accurate.      
Sec3_2020_11_16_12_52.tex:Each ensemble member is then described by $4^3=64$ times less mesh elements than the single simulation on the fine grid. If one considers that one main simulation and $100$ ensemble members are run simultaneously, and if calculation times are normalized over the main simulation, this implies that $R_\text{RAM} = 1 + 100/64 = 2.56$ i.e. the total cost in RAM is increased to just $2.56$ times the cost of the classical simulation. \lc{Pourquoi le 1 devant ?}
Sec3_2020_11_16_12_52.tex:For $r_\text{C}=8$, the RAM requirement is $R_\text{RAM}=1+100/8^3=1.195$, thus just a $20\%$ increase in RAM requirements. \lc{phrase pas clair}
Sec3_2020_11_16_12_52.tex:This is clearly orders of magnitude more advantageous than a fine-grid classical EnKF application with $N_\text{e}=100$, since in this case $R_\text{RAM}=N_\text{e}=100$.\lc{je ne comprends pas}  
Sec3_2020_11_16_12_52.tex:\item[-] Owing to the iterative procedures of steps $4$ and $5$, regularization \lc{dans quel sens ?} of the final solution is naturally obtained. 
Sec3_2020_11_16_12_52.tex:However, in this case, no regularization \lc{dans quel sens ?} is obtained unless specific corrections are included. 
Sec3_2020_11_17_09_43.tex:The multigrid-ensemble algorithm works through the steps described below. In the following description, the notation $\mathbf{\Psi}$ might hold for both $\mathbf{\Psi}$ and $\widetilde{\mathbf{\Psi}}$ introduced in \eqref{eq:generalDiscretizedFormInt}, depending on the choice of the time integration strategy. Note that the states $\left(\mathbf{x}^\text{C}_{k}\right)^{*}$ and $\left(\mathbf{x}^\text{C}_k\right)^{'}$ are associated to the single fine-grid simulation only and are natural to the FAS multigrid method described before. They represented the projection on the coarse-grid of the first fine-grid solution ($\left(\mathbf{x}^1\right)^\text{C}$ in the FAS algorithm) and the coarse-grid solution obtained with an iterative process starting from the first fine-grid solution projected on the coarse grid ($\left(\mathbf{x}^2\right)^\text{C}$ in the FAS algorithm), respectively. $\left(\mathbf{x}^\text{C}_k\right)^\text{e}$ represents an intermediary estimated-state used to calculate $\left(\mathbf{x}^\text{C}_k\right)^{'}$.  
Sec3_2020_11_17_09_43.tex:\item \textbf{First iteration on the fine grid}. Starting from an initial solution on the fine grid $\left(\mathbf{x}^\text{F}_{k-1}\right)^\text{a}$, an iterative procedure is applied to obtain a forecast state $\left(\mathbf{x}^\text{F}_{k}\right)^\text{f}$. A residual $\mathbf{\delta}^\text{F}$ is calculated.
Sec3_2020_11_17_09_43.tex:\item \textbf{Time advancement of the ensemble members}. $\mathbf{\Psi}^\text{C}$ is used to determine the state matrices $\left(\mathbf{\Psi}\right)^{\text{C},(i)}$ \lc{je ne vois pas de quoi tu parles} for the advancement in time of the $N_\text{e}$ ensemble members defined on the coarse grid. Note that the forecast model used for every ensemble member is the same, i.e. Navier-Stokes, but the discretization process (contained in $\mathbf{\Psi}$) is unique for each member, thus the superscript $i$ in $\left(\mathbf{\Psi}\right)^{\text{C},(i)}$. The ensemble forecast $\left(\mathbf{x}^\text{C}_{k}\right)^{\text{f},(i)}$ is corrected with the standard Dual EnKF procedure to obtain $\left(\mathbf{x}^\text{C}_{k}\right)^{\text{a},(i)}$ as well as the parametric optimization.
Sec3_2020_11_17_09_43.tex:\item \textbf{Determination of the state variables on the coarse grid}. If observations are not available, the state $\left(\mathbf{x}^\text{C}_k\right)^{'}$  \lc{de quoi tu parles ?} ($\left(\mathbf{x}^2\right)^\text{C}$ in the FAS algorithm) is obtained using the classical multigrid procedure. On the other hand, if observations are available, the ensemble error covariance matrix $\left(\mathbf{P}_k^\text{C}\right)^{\text{f},\text{e}}$
Sec3_2020_11_17_09_43.tex: is used to determine the state estimation $\left(\mathbf{x}^\text{C}_k\right)^\text{e}$. In practice, $\left(\mathbf{x}^\text{C}_k\right)^\text{e}$ corresponds to the initial state $\left(\mathbf{x}^\text{C}_{k}\right)^{*}$ plus a standard Kalman Filter correction obtained with the observation and the ensemble statistics.  \lc{de quoi tu parles ?}. The state estimation is used as initial condition in the coarse-grid iterative process in order to obtain $\left(\mathbf{x}^\text{C}_k\right)^{'}$ \lc{de quoi tu parles ?}. $\left(\mathbf{x}^\text{F}_k\right)^{'}$ \lc{de quoi tu parles ?} is then updated using the results obtained on the coarse space: $\left(\mathbf{x}^\text{F}_k\right)^{'}=\left(\mathbf{x}^\text{F}_{k}\right)^\text{f}+\Pi_\text{F}\left(\left(\mathbf{x}^\text{C}_k\right)^{'}-\left(\mathbf{x}^\text{C}_{k}\right)^{*}\right)$.
Sec3_2020_11_17_09_43.tex:Two different levels of representation (fine and coarse grids) are used to obtain a data-driven fine grid estimation.\todolc{Changer la notation des projecteurs.}\lc{je ne comprends pas cette figure}}
Sec3_2020_11_17_09_43.tex:\item[-] As previously stated, $\mathbf{\Psi}^\text{C}$ and its role in the determination of the matrices $\left(\mathbf{\Psi}\right)^{\text{C},(i)}$ is an essential step in the MEnKF strategy. In non-linear problems of interest in fluid mechanics, the state transition model $\mathbf{\Psi}$ includes information of the multi-scale interactions that are specific for every case investigated. The simplest possible choice, which is the one adopted in this work, is to calculate the coefficients of the matrices $\mathbf{\Psi}^\text{C}$ and $\left(\mathbf{\Psi}\right)^{\text{C},(i)}$ separately for each simulated state. Thus, the similarities between the employed state matrices are limited to the use of the same discretization schemes / structure of $\mathbf{\Psi}$. However, one can envision to use the non-linear information conserved in $\mathbf{\Psi}^\text{C}$, which is supposedly accurate, to improve the accuracy of the prediction of the ensemble members. This aspect is discussed in the perspectives included in Sec.~\ref{sec:conclusions}.
Sec3_2020_11_17_09_43.tex:However, these corrections may result in an increase of the computational resources required. Here, the multigrid algorithm itself is used for regularization (i.e. smoothing the discontinuities in the physical variables produced by the update via Kalman Filter) \lc{dans quel sens ?} of the flow. In fact, if an intentionally reduced tolerance is imposed in the iterative steps $4$ and $5$, the final solution will keep memory of the features of the state estimation produced in step $3$. However, the iterative resolution will smooth the estimation via the state transition model $\mathbf{\Psi}$, which will perform a natural regularization \lc{dans quel sens ?} of the flow. Clearly, if a reduced tolerance is imposed, the final solution will not necessarily respect the conservativity constraints of the model equations. However, one can argue that complete conservativity is not an optimal objective in this case, if the model state at the beginning of the time step is not accurate.      
Sec3_2020_11_17_09_43.tex:Each ensemble member is then described by $4^3=64$ times less mesh elements than the single simulation on the fine grid. If one considers that one main simulation and $100$ ensemble members are run simultaneously, and if calculation times are normalized over the main simulation, this implies that $R_\text{RAM} = 1 + 100/64 = 2.56$ i.e. the total cost in RAM is increased to just $2.56$ times the cost of the classical simulation. \lc{Pourquoi le 1 devant ?}
Sec3_2020_11_17_09_43.tex:For $r_\text{C}=8$, the RAM requirement is $R_\text{RAM}=1+100/8^3=1.195$, thus just a $20\%$ increase in RAM requirements. \lc{phrase pas clair}
Sec3_2020_11_17_09_43.tex:This is clearly orders of magnitude more advantageous than a fine-grid classical EnKF application with $N_\text{e}=100$, since in this case $R_\text{RAM}=N_\text{e}=100$.\lc{je ne comprends pas}  
Sec3_2020_11_17_09_43.tex:\item[-] Owing to the iterative procedures of steps $4$ and $5$, regularization \lc{dans quel sens ?} of the final solution is naturally obtained. 
Sec3_2020_11_17_09_43.tex:However, in this case, no regularization \lc{dans quel sens ?} is obtained unless specific corrections are included. 
Sec4.tex:This also implies that the total number of nodes employed to perform the calculation is $N_x=800$.  
Sec4.tex:\lc{reprendre ICI}
Sec4.tex:Results are now investigated for increasing values of $r_\text{\tiny C}$. Results for $r_\text{\tiny C}=8$ are shown in Fig.~\ref{fig:MgENKF_states_rc8}. Minor differences between the state estimation and the true state can be observed in this case. This discrepancy is due to the lack of resolution of the ensemble members. In fact, the resolution in this case is of $10$ mesh elements per characteristic length. This number of points is arguably not enough to provide an accurate representation of the sinusoidal waves which are imposed at the inlet. However, one can see that no spurious numerical effects are observed as the estimator provides a smooth, continuous prediction of the velocity. The discrepancy between the true state and the state estimation is mainly associated with an erroneous calculation of the Kalman Gain due to the under-resolution of the ensemble, which also affects the parameter estimation. A combined analysis of Fig.~\ref{fig:amplitude_avg_DENKF} and \ref{fig:MgENKF_states_rc8} shows that, due to the lack of accuracy in the estimation of $\theta_1$, the variable $u$ is over-predicted for $t < 2 t_c$ while it is slightly under-predicted for $t > 4 t_c$.    
Sec4.tex:This aspect is further investigated considering the computational resources required to perform a full assimilation window for each $r_\text{\tiny C}$ value. In Fig.~\ref{fig:calc_time_burgers} results are shown and normalized over the case $r_\text{\tiny C}=1$. One can see that the computational resources required rapidly decrease with increasing $r_\text{\tiny C}$, even for this simple one-dimensional test case. For large values of $r_\text{\tiny C}=8,16$ one can see that the computational resources reach a plateau. Here the computational time to perform the DA procedures, which is the same for every $r_\text{\tiny C}$, is of similar order of magnitude of the calculation for the time advancement of the ensemble members.
Sec4.tex:\includegraphics[width=1\textwidth]{figures/calc_time.png}
Sec4.tex:\caption{\label{fig:calc_time_burgers}
Sec4.tex:\lc{que gagne-t-on à passer en log sur les abscisses ?}
Sec5.tex:The sinusoidal behaviour of the velocity at the inlet is characterized by a constant frequency $f_c=1/t_c$ with $\omega=2\pi f_c$. However, the time-varying amplitude of the sinusoidal wave is driven by the parameter $\theta(t)=\theta_0(1+sin(\omega_{\theta} t))$, where $\theta_0$, $\omega_{\theta}=f_c/b$ and $b$ are constants. The density at the inlet is fixed $\rho(x=0,t)=\rho_0$ as well as the total energy $E(x=0,t)=E_0$, which is calculated as $E_0=\frac{1}{\gamma-1}\frac{p_0}{\rho_0}+0.5 u_0^2$. The outlet boundary condition is extrapolated from the nearest points to the outlet. The initial condition imposed for $t=0$ is $u(x,t=0)=u_0$, $\rho(x,t=0)=\rho_0$ and $E(x,t=0)=E_0$ everywhere in the physical domain. The fluid is an ideal gas with $\gamma=1.4$, $\rho_0=1.17$ and $T_0=300$ in S.I. units. Note that from now on the units
Sec5.tex:The computational domain has been set to a size of $L_x=10$. A uniform mesh distribution is used for every calculation. Similarly to the analysis in Sec.~\ref{sec:Burgers1D}, $80$ mesh elements are used to discretize a characteristic length $\lambda$ for a total of $N_x=800$ elements in the domain. Finally, the normalized value of $\Delta t$ is set to $\Delta t=0.0006$.
Sec5.tex:The results for the estimation of the time-varying parameter $\theta$ are reported in Fig.~\ref{fig:parameter_euler}. The three analyses performed are able to capture the time evolution of $\theta$. This is an important result, considering that no a priori information was provided for the evolution of this parameter. A more detailed analysis reveals a lag in the parameter estimation. The application of a simple Kalman Filter is responsible for this observation, while a Kalman Smoother (KS) should have been used to obtain a better synchronization. However, considering that implementation of KS is straightforward in this case and that observation is always provided close to the inlet, we decided that the increase in required resources by the KS were not justified. The lag is increased when a relatively small number of DA analyses is performed. One can see that the prediction is significantly degraded for $f_a=2$, while similar results are obtained for $f_a=10,55$. In addition, $\theta$ tends to be underestimated (around $10\%$) when it reaches its maximum value. This result is arguably associated with the under-resolution of the coarse level of the grid, where the gradients of physical variables are calculated with lower accuracy.
Sec5.tex:Now, results dealing with the State Estimation are discussed. The predicted physical variable $\rho u$, normalized over the initial value $\rho_0 u_0$, is shown in Fig.~\ref{fig:MGENKF_states_rc4_euler_f2}, \ref{fig:MGENKF_states_rc4_euler_f10} and \ref{fig:MGENKF_states_rc4_euler_f55} for $f_a=2,10,55$. The lack of an exact estimation of the parameter $\theta$ produces different results depending on the value of $f_a$ considered. For the $f_a=2$ case, the state estimation is significantly distant from the truth. It appears that the field correction applied via the Kalman gain is not able to compensate the poor estimation of $\theta$. However, accurate results are observed for $f_a=10,55$. Even though the parameter optimization of $\theta$ is not exact, the total state estimation including the correction via Kalman gain is very precise. For the case $f_a=55$ almost no discernible difference is observed between the state estimation and the truth. %This test-case is representative of the functioning of the MEnKF algorithm. %There are two levels of correction on the fine grid directly affected by the coarse grid ensemble. The first level of correction is provided by the parameter optimization process. A second level of correction is obtained by means of direct state correction on the fine grid, which is performed using the kalman gain calculated from the coarse ensemble.
Sec5.tex:  \caption{\label{fig:MGENKF_states_rc4_euler_f2} Time evolution of the momentum $\rho u$ normalized by $\rho_0u_0$, calculated using the Multigrid EnKF (MEnKF) estimator. The case for $f_a=2$ is here shown. Results are shown for (a) $t=1.23$, (b) $t=8.32$ and (c) $t=16.30$ (in $t_c$ units). The black and the grey line represent the true and estimated states, respectively.}
Sec5.tex:  Time evolution of the momentum $\rho u$ normalized by $\rho_0u_0$, calculated using the Multigrid EnKF (MEnKF) estimator. The case for $f_a=10$ is shown. Results are shown for (a) $t=1.23$, (b) $t=8.32$ and (c) $t=16.30$ (in $t_c$ units). The black and the grey line represent the true and estimated states, respectively.}
Sec5.tex:  \caption{\label{fig:MGENKF_states_rc4_euler_f55} Time evolution of the momentum $\rho u$ normalized by $\rho_0u_0$, calculated using the Multigrid EnKF (MEnKF) estimator. The case for $f_a=55$ is here shown. Results are shown for (a) $t=1.23$, (b) $t=8.32$ and (c) $t=16.30$ (in $t_c$ units). The black and the grey line represent the true and estimated states, respectively.}
Sec6.tex:The numerical algorithm is used to analyse the two-dimensional spatially evolving mixing layer for $Re=100$. For this Reynolds number the flow exhibits unsteady features. In addition, the characteristics of the mixing layer are strongly affected by the inlet and, in particular, by \textit{ad-hoc} time perturbations imposed \cite{Ko2008_pof,Meldi2012_pof}. The computational domain has been set to a size of $14\Lambda\times 6\Lambda$ in the streamwise direction $x$ and normal direction $y$, respectively. The characteristic length $\Lambda$, which is taken as reference length  from now on, is calculated as $\Lambda=A\delta_0$, where $\delta_0$ is the initial vorticity thickness imposed at the inlet. In this case, $A=14.132$ for the most unstable wavelength obtained through the Linear Stability Theory (LST) for $Re=100$. The mesh resolution in the horizontal direction is constant for $x \leq 10$ and the size of the elements is $\Delta x = \frac{\delta_0}{8}$. For $x \geq 10$ a sponge zone is established with a coarsening ratio between successive elements which increases from $1.025$ to $1.04$. The resolution in the normal direction is constant and equal to $\Delta y=\frac{\delta_0}{20}$ for $-0.18\leq y \leq 0.18$. Outside this zone, the mesh elements increase in size moving away from the centerline with a constant coarsening ratio of $1.01$.     
Sec6.tex:The Reynolds number of the flow is calculated as $Re=(U_1-U_2)\delta_0/\nu=100$ with asymptotic velocities set to $U_1=173.61$ and $U_2=104.17$, which correspond to a Mach number $Ma=0.5$ and $Ma=0.3$, for each stream respectively. The kinematic viscosity and thermal diffusivity of the flow are considered to be constant and their value is fixed to $\nu=1.568\times 10^{-5}$,  $\alpha=22.07\times 10^{-7}$. All the quantities here introduced are expressed in S.I. units. 
Sec6.tex:  \caption{\label{fig:2D-mxl-trutht10} Flow calculated using a 2D compressible Navier-Stokes equation. Visualization of the normal momentum $\rho v$ for the reference simulation for $t=10$. In sub-figure $(a)$, $\epsilon_1$ is constant whereas in $(b)$ it is time-varying.}
Sec6.tex:As expected $\Gamma_k^\text{\tiny F}=0$ everywhere for the third case (\textit{i.e.} parameter estimation only). Here the time advancement of the solution is performed using the model only, which exactly complies with the discretized equation and respects conservativity (up to a convergence error which is negligible). On the other hand, results in Fig.~\ref{fig:GAMMA} (a) show some lack of conservativity in the physical domain for the first described case. This is also expected, because no constraint is imposed to force the Kalman gain correction to comply with the dynamic equations. Finally, results for the MEnKF are shown in Fig.~\ref{fig:GAMMA} (b). The topology of $\left(\Gamma_k^\text{\tiny F}\right)^*$ is here very similar to the results observed for the first described case. However, one can clearly see that this field appears to be sensibly smoothed out by the multigrid iterative procedures in step 4 and 5 of the MEnKF algorithm. As previously discussed, complete conservativity starting from an erroneous state at $k-1$ is possibly not an optimal objective, while one wants a regularized solution to avoid affecting the precision of the global calculation. On this last objective, the MEnKF appears to provide a better result when compared with the classical EnKF, described in the first case. Considering also that the MEnKF showed better accuracy than the algorithm relying on parameter estimation only, one can conclude that the MEnKF provides an efficient compromise between global accuracy and regularization of the solution. In order to draw more information about this important aspect the MEnKF tool needs to be tested for the simulation of three-dimensional compressible flows, where the Kalman gain correction may be responsible for important acoustic phenomena which are not observable in 2D and 1D dynamic systems.   
Sec7.tex:A sequential estimator based on a Kalman filter approach for Data Assimilation of fluid flows is presented in this research work. This estimator exploits iterative features which are employed in several CFD codes for the resolution of complex applications in fluid mechanics. More precisely, the multilevel resolution associated with the multigrid iterative approach for time advancement is used to generate several low-resolution numerical simulations. These results are then employed as ensemble members to determine i) the correction via Kalman filter, which is then projected on the high-resolution grid to correct a single simulation which corresponds to the numerical model and ii) an optimization of the free parameters driving the simulation. One of the main advantages of the model is that, owing to the iterative procedure for the calculation of the flow variables, the final solution is regularized.
SecAbstract.tex:%\todolc{à modifier en phase finale}
SecAbstract.tex:A sequential estimator based on the Ensemble Kalman Filter for Data Assimilation of fluid flows is presented in this research work. The main feature of this estimator is that the Kalman filter update, which relies on the determination of the Kalman gain, is performed exploiting the algorithmic features of the numerical solver employed as a model. More precisely, the multilevel resolution associated with the multigrid iterative approach for time advancement is used to generate several low-resolution numerical simulations. These results are used as ensemble members to determine the correction via Kalman filter, which is then projected on the high-resolution grid to correct a single simulation which corresponds to the numerical model. The assessment of the method is performed via the analysis of one-dimensional and two-dimensional test cases, using different dynamic equations. The results show an efficient trade-off in terms of accuracy and computational costs required. In addition, a physical regularization of the flow, which is not granted by classical KF approaches, is naturally obtained owing to the multigrid iterative calculations. The algorithm is also well suited for the analysis of unstationary phenomena and, in particular, for potential application to in-streaming Data Assimilation techniques.  

